What Do Developers Ask About ML Libraries? A Large-scale Study Using Stack Overflow

Modern software systems are increasingly including machine learning (ML) as an integral component. However, we do not yet understand the difficulties faced by software developers when learning about ML libraries and using them within their systems. To that end, this work reports on a detailed (manual) examination of 3,243 highly-rated Q&A posts related to ten ML libraries, namely Tensorflow, Keras, scikit-learn, Weka, Caffe, Theano, MLlib, Torch, Mahout, and H2O, on Stack Overflow, a popular online technical Q&A forum. We classify these questions into seven typical stages of an ML pipeline to understand the correlation between the library and the stage. Then we study the questions and perform statistical analysis to explore the answer to four research objectives (finding the most difficult stage, understanding the nature of problems, nature of libraries and studying whether the difficulties stayed consistent over time). Our findings reveal the urgent need for software engineering (SE) research in this area. Both static and dynamic analyses are mostly absent and badly needed to help developers find errors earlier. While there has been some early research on debugging, much more work is needed. API misuses are prevalent and API design improvements are sorely needed. Last and somewhat surprisingly, a tug of war between providing higher levels of abstractions and the need to understand the behavior of the trained model is prevalent.

==> Intra.tex <==
\paragraph*{\textbf{Libraries that use uncommon or new formats of 
		data create difficulties in data preparation.}}

We can observe in \figref{fig:interlib} that the developers using
\weka and \mllib library face more difficulty in the data preparation 
stage while adapting data to the ML Library. 
For \weka 36/127 questions and for \mllib 41/123 focused on data 
preparation issues.
%\input{ob1}
%As we observe in a sample question in Figure \ref{fig:ob1weka} that the user is
%trying to use a dataset from a well-known ML dataset repository \cite{uci}. 
%Usually these datasets are preprocessed to do machine learning and
%importing these datasets can be done directly. But an user of \weka user is not
%able to successfully adapt the dataset to the library for training due to the
%failure of conversion to ARFF format needed by the library. 
Similarly, developers using Apache Spark \mllib also have a higher percentage of difficulties
during the data preparation stage because it uses RDD format of data
which is a less popular format. Adapting the data for the library,
converting from popular data formats to the format required or preferred by the
library are some common problems faced by the users when the library uses less
popular data formats. 
%We have studied and labeled 127 \sof questions on \weka and 
%found 36 of them is about data preparation. 
%And questions out of 123 questions in \mllib 41 are about data preparation. 

\paragraph*{\textbf{Built-in feature selection library doesn't mean 
		improved feature selection functionality.}}
As an example, 
\scikit library provides a rich set of functionalities for feature selection and feature extraction, but we found a number of questions about feature selection for this library. 
For Scikit, 70/849 questions were about feature selection/extraction.
%An example of such question is shown
%in \figref{fig:ob2sklearn}. 
%\input{ob2}
% For example, in Figure \ref{fig:ob2sklearn} the user is facing some 
% problem in using the built-in API to select features from the data 
% for building a model. 
Users also face difficulties in encoding data, cleaning data, shuffling 
and splitting of data, extracting features from data, data cleaning, etc.
Most of these queries have developers wondering about an exception or 
an unsatisfactory result. 
% We have studied 849 \scikit questions and found that 70 questions 
% of those are about feature selection/extraction. 

\paragraph*{\textbf{Libraries that use opaque higher abstraction create an additional difficulty for users in model creation. }}
Some libraries hide all of the details of building ML models from the developer. 
That makes using the library easier for average developers but can 
also be a source of difficulties for the developer because they don't 
have an insight into the failures in constructing the model or in the 
performance of the model.
For \scikit 175/849 questions, and for \keras 94/385 questions were 
about this topic.
%\figref{fig:ob3} shows an example where a developer is trying to use the APIs provided by the library to build a model but is getting an error in building the model correctly. 
%\input{ob3}
This problem is more common among the developers using \scikit and \keras. 
These two libraries abstract away almost all of the details from the developers. 
% We have found that 175 questions out of 849 in \scikit and 
% 94 questions out of 385 in \keras are about model creation. 

\paragraph*{\textbf{Debugging and monitoring facilities are absent in general.}}
Lack of rich and interactive debugging tools makes building ML models difficult.
A number of problems faced by developers, e.g. 
when a model is throwing an exception at training time, a model is 
not converging or learning as the iteration of training goes on, 
a model is not predicting well, model creation is not correct 
and producing incorrect results, a model is not performing well for 
a particular instance of a problem, etc, can be minimized to a great 
extent with effective debugging tools.
Fortunately, some recent work has started to address these 
issues~\cite{chakarov2016debugging,tdebug}, but much more work 
is needed. 
Due to the lack of debugging and tools to monitor pipeline causes of failure are hard to identify. 
%While studying the questions we have found that a lot of those 
%questions are asked here because of the absence of debugging 
%and pipeline monitoring. 
% \tensor team has attempted to add debugging options through TensorDebug \cite{tdebug}. The concept of debugging some tasks by implementing machine learning with the help of probabilistic programming is presented by the authors in \cite{chakarov2016debugging}.

\paragraph*{\textbf{\tensor users face less difficulty in data 
		preparation stage due to tensor usage}}
Surprisingly, \tensor has comparatively fewer difficulties in data preparation. There are some difficulties in adapting TFRecords (a data format used by \tensor) or storing data in this format. 
This could be because this ML library provides multiple adapters 
to read and store data.
In \tensor, the dataset is stored as elements of same size and each element can contain one or more Tensor objects. 
Each Tensor object also has type information and shape information added to it. 
Using Tensor objects and providing functionalities to read raw data and forming dataset using Tensor objects reduces errors, adaptation and data cleaning related problems. 
An example of how the dataset is represented as a tensor from a random uniform matrix of 4*10 size is given in the following code snippet:
\input{tensor}
We see that the dataset is read and parsed as tensor by the library with type and shape information. 
The library enables easier adaptation of data as well as debugging any dataset related problem by tensor debug. 
\torch and \theano also use tensors as their data structure. 
Although they have comparatively few problems in the data preparation stage, the data adaptation and loading APIs create slightly more difficulties compared to \tensor in these libraries. 
For \tensor 234/1318 questions were about data preparation that is proportionally lower compared to other libraries.
% We have studied that 234 questions out of 1318 questions are about data preparation. 
% Which is proportionally lower than other popular libraries.

%\paragraph*{\textbf{Debugging and runtime monitoring can make a library more
%		appealing to the developers}} \tensor popularity is growing very fast since the
%inception of the library in November 2015. It provides some model evaluation and
%monitoring of the model at runtime through a visual interface using TensorBoard.
%It also provides some debugging functionality using TensorDebug, which uses Tensor
%data structure to represent its data internally and flow data to different
%components in the pipeline. 
%The interest in these features is evident, and developers also have questions
%about the handling of sparse tensor data that is not currently supported. 
%In \tabref{tbl:dataset}, almost 50\% questions with $S \geq 0$ 
%are about \tensor.
%%Its developers have some questions on handling
%%sparse tensor data. And the monitoring of sparseness of the tensor at different
%%stage is not yet supported. Analysis of sparsity of tensors at different stages
%%of the pipeline and then optimizing the computation can be future work. And also
%%the storing technique of different types of sparse tensors can be a great
%%addition. Some research on the line has been proposed and presented by Kjolstad 
%%{\em et. al.}~\cite{kjolstad2017tensor}.
%Its developers have some questions on handling
%sparse tensor data. And the monitoring of sparseness of the tensor at different
%stage is not yet supported. Analysis of sparsity of tensors at different stages
%of the pipeline and then optimizing the computation can be future work. And also
%the storing technique of different types of sparse tensors can be a great
%addition. Some research on the line has been proposed and presented by Kjolstad 
%{\em et. al.}~\cite{kjolstad2017tensor}.

\paragraph*{\textbf{Interoperability of models across libraries is needed}}
Converting models trained using one library and using it with another library is a
common problem. For example, let's consider someone has trained an SVM model on a
particular dataset D. The user then wants to load the model in \weka and use that
for future prediction. Some libraries provide support to convert model for
use with other libraries but such support isn't always adequate. 
The developers often have questions about reusing trained model with other platforms. 
Out of 61 questions in \torch, we found 3 questions requesting help to convert 
model to reuse in another library, 4 out of 127 in \weka, 3 out of 132 in \caffe 
asks help with ML model reuse.

\paragraph*{\textbf{Choice of the model needs recommendation support}}
All the library users face comparatively higher difficulty in model creation than other subcategories. 
Deep learning library users have comparatively more difficulty in the model creation stage. 
Almost 30\% of the questions asked by deep learning library users on 
\sof, where the score is at least 5 is on the choice of model. 
This suggests the need to develop recommendation systems to address this need.
% Model of choice contains topics related to model creation, selecting best model, 
% converting model etc. This suggest applying software engineering research 
% applying concepts of meta learning \cite{vilalta2002perspective} to help the 
% framework suggest the path and throw warnings and feedback.

\paragraph*{\textbf{Libraries that provide more optional parameters complicate hyperparameter tuning}}
Hyperparameter tuning related questions are comparatively frequent among the
\scikit users. Usually, \scikit APIs take a lot of optional parameters.
For example, we see an API to create \texttt{AdaBoostClassifier} below with 5 optional
parameters initialized to some default values. 
\input{sklearn} 
The best\_estimator is set to None but the user may need to choose an estimator to
get the best performance. Learning rate is by default set to 1.0. At this
learning rate, it is highly likely that the model will not learn anything. So the
user may often use these APIs incorrectly and wonder why ML model is
not producing the useful result. Since these are optional parameters, the user will not even get any error or warning. Finding good values for these parameters and tuning them to make the best model, avoiding over-fitting are frequent questions among developers using \scikit. There have been some 
Github issues filed to the repository of \scikit as bugs 
(See \figref{fig:tune} for an example)
but the underlying problem was that the developer was not able to trace why the model is not showing expected accuracy, and unable to tune hyperparameters. We have found 36 questions out of 849 in \scikit asking help about hyperparameter tuning.


\input{tune}

%\paragraph*{\textbf{Abstraction $\neq$ successful developers}}
%\keras and \scikit are highly abstract and hide all the details of machine
%learning implementations from the users. This sometimes creates some untraceable
%suboptimal performance in prediction as well as fatal errors. Because the user
%doesn't have the way to trace where the model was not functioning correctly,
%whether some over-fitting problem happened. For example an user has built a
%model successfully and got training successful with satisfactory training
%accuracy. But when the new data is given input to the model for prediction the
%prediction accuracy is very low. In most of these cases the user even doesn't
%have any way to trace the reason of these sub-optimal performance. So
%abstracting the functionalities and making more general users to practice
%machine learning doesn't ensure that they are doing machine learning with
%satisfactory success.

\paragraph*{\textbf{More abstract deep learning libraries have more runtime error}}
In \keras, a highly abstract deep learning library, developers get the comparatively higher error at runtime. 
\input{keraserr}
For example in Figure \ref{fig:ob6} a developer has built the model successfully
yet they get an error at runtime. The reason is that model building in deep
learning model needs to successfully connect multiple hidden layers along with
the input and output layer. But with abstract libraries, the user doesn't have
any tools to inspect within the model.
Furthermore, while connecting these APIs to build the neural network the 
user has many places of single point failure starting from dimension mismatch, 
wrong activation function usage as well creating hidden loops with 
a performance overhead. 20 out of 385 questions for \keras are about training 
time error 
We have found 20 questions related to training time error out of 385 questions in \keras. 

\paragraph*{\textbf{Model creation appears to be harder for parallel ML libraries}}
The libraries that are specialized for doing machine learning in the cluster 
have more difficulties in the choice of model phase, especially in model creation subcategory. 
\input{mahout}
For example, the users of \mllib and \mahout face higher difficulties in model creation, 
running model in parallel following map-reduce paradigm, selecting the appropriate model.
\figref{fig:mahout} shows an example. 
For \mllib and \mahout 33/123 and 21/64 questions focus on this issue.
%To illustrate see \figref{fig:mahout} where the developer is trying to build a model to
%build his custom model but he is facing difficulty to use the library on
%creating that model. The top voted answer suggested how can the person achieve
%his goal by combining multiple ideas as well as how the performance can be
%optimized using to make the best use of the cluster. We have seen two popular
%libraries for cluster \mllib and \mahout have respectively 33 out of 123 and 21
%out of 64 questions on model creation.

\paragraph*{\textbf{Dependence of model creation on multiple files can be the
		cause of more failure}} \caffe users have problems in model creation due to the
dependency of the model on multiple files. To create a model successfully one
needs to make a schema file in protobuf format, create a solver file and write
codes in c++ or python to build the model. For example, this tutorial
\cite{caffetutorail} describes multiple separate components in separate files
needed to build a model successfully using \caffe and Python. This gives us some
intuition that the framework where the model depends on multiple things or there
are more than one way of creating the same model creates technical challenges in
the model creation phase. 
% \caffe is mainly used for deep learning and was
% developed by Berkley Vision. 
The \caffe models are defined in a plain text protocol
buffer schema (prototxt), which adds to the complexity of using this library to
many users. A lot of questions on \caffe in \sof are about
successfully creating the schema in the prototxt file and the reason of the
failure of a model defined using prototxt file. In our study we have seen 36 out
of 135 \caffe questions are about model creation problems.

\paragraph*{\textbf{API misuse in ML needs deeper exploration}}
The ML libraries have APIs that are very often misused. 
The general guideline of API design is such that it should be difficult to 
misuse the API \cite{bloch2006design}.
But we have seen a lot of the problems faced by developers are due to 
using the API in an improper way.
This problem happens in the APIs at almost all stages of the pipeline 
starting from data preparation to prediction. 
\input{apimis}
For example, we see in Figure \ref{fig:apimis}a a question asked by a user that,
his training takes much time or longer number of iterations to get a certain
training accuracy. In one API he is able to achieve the accuracy only in 5
iterations where in the other API the user needs 60 iterations to reach the same
accuracy. The library is working fine, without any error and eventually reaching
the same accuracy. But still, the user is puzzled by almost 12 times
higher number of iterations in using the second API. And the answer in Figure
\ref{fig:apimis}b suggests that the second API needs the data to shuffled
properly before passing to the API in every iteration. And changing only that
part solves the performance problem. 
This is an example of API misuse where the precondition of the second API 
is not satisfied which leads to a performance bottleneck.
% So here a misuse of API is being occurred
% without satisfying preconditions and causing a performance bottleneck. 
For another example, let's consider a problem related to the creation of a
NaiveBayes model. Only a part of the code snippet where API misuse occurred is
shown below:
\input{sklearnapi}
The code failed to work successfully giving dimension mismatch error in 
some parts of the code. 
The solution to the problem is in properly using the API $csr\_matrix()$. 
The API needs to have a shape parameter defined explicitly and the correct 
way to use the API is to explicitly defining the shape shown in the following code.
\input{correction}
Let's study another kind of API misuse happening due to API update by the 
library providers. 
The following piece of code was working in Apache Spark \mllib before 
Spark version 2.0. 
Since Spark version 2.0 this API is not working and the user doesn't 
have any idea what happened overnight. 
This is one of the top voted questions on Apache Spark \mllib category.
\input{rddapi}
Since version 2.0 the Line 3 became invalid and the valid line is following
\input{valid}
We have found that similar version incompatibility problems are also 
prevalent in other ML libraries.

Besides the API misuse scenarios discussed above, many other kinds of API 
misuse are common in ML libraries, and a more detailed analysis and categorization
of errors is needed (much like MUBench~\cite{Amann2016}). 
Some common problems include failure to find important features, 
improperly preparing the dataset, performance, over-fitting problems,
suboptimal prediction performance, etc. 
A detailed analysis of API misuse is beyond the scope of this work.
% It causes problems on the failure to find important features, properly preparing
% the dataset, performance, over-fitting, suboptimal prediction performance,
% error, warnings etc. We leave it to explore in details by classifying the API
% misuse happening in machine learning library usage and studying them thoroughly
% as a future work.

\paragraph*{\textbf{Shape mismatch is another problem where tensor or matrix
		dimensions between layers become a concern}} Shape mismatch of tensors at
different layers is also a common problem among the libraries that use tensors
or matrices. This problem is seen more commonly in deep learning libraries. For
example, when tensors pass from layer $i$ to layer $j$ in the network then there
should be some size compatibility otherwise the library can raise an exception during
training or fail during prediction.
\input{shape}
For example, see \figref{fig:shape} that has a sample question on shape
mismatch. In \tensor library, 40 out of 1318 questions are about shape mismatch.

\paragraph*{\textbf{Type mismatch errors are common}} 
Type mismatch is also a common problem faced by developers. 
The training fails due to this type mismatch problem. 
\input{type}
For example Figure \ref{fig:type} shows a question on type mismatch. 
The whole training process failed in the middle where the library found an unwanted type.

\paragraph*{\textbf{Data preparation remains a major challenge for ML libraries}} 
We observe a generally higher number of questions about the data
preparation stage. Data cleaning related problems can often lead to failure in
training. Feature extraction, feature selection, adapting and preparing the
data through encoding, shuffling needs to be added with the library and needs to
be user-friendly. We have seen all the
libraries have 25\%-30\% of questions about data preparation
stage and consists of almost one-third of the total questions.

\paragraph*{\textbf{Static and dynamic analysis support is sorely needed}}
Static and dynamic analysis (or even more capable typechecking) can resolve a
lot of issues related to shape mismatch, type mismatch, and others. But current
libraries lack any verification features. To illustrate, let us observe the
following \keras code:
\input{kerasstatic} 
The reason for the failure of the model is Line 8 $input\_shape$. The accepted
answer suggests that shape should be $(32,1)$ instead of $(32,3)$. The user
could not verify statically whether the built network is matching in shape, is there any
port unconnected or extra port while building the architecture. If we have the
tools that could tell the developer that, using dimension (32,1) can cause 2
out of 3 ports of the next layer to be unconnected then it would be much easier
for the developer to find these errors themselves. A lot of these errors can be
detected by program analysis support and by providing feedback to the users. 
In fact, a lot of these high scores questions call for richer analysis features.
% can turn out to be a silly question to be
% downvoted when the user gets these tools in hand.


==> Result.tex <==
\subsection{Result}
In this section we present our findings from the analyses to answer the research questions. 

\textbf{RQ1:}  What stages are more difficult in ML pipeline? \newline
Our analyses presented previously reveals the answer to which on is the most difficult stage in ML pipeline. 
Somewhat expectedly the model creation is the most difficult, but surprisingly data preparation is the next difficult stage which turns out to be more difficult than training stage.
\findings{Model creation is the most challenging (yet critical) in ML 
	pipeline, especially for libraries supporting distributed ML on 
	clusters like \mahout and \mllib. 
	%with 43.75\% and 23.52\% questions, respectively. 
	%\mahout is an outlier in this step. 
}{This calls for tool support in creating models, 
	especially in distributed machine learning.} 
Our analyses also shows trying to use multiple languages for configuring the model creates additional complexity. 
\findings{Multilingual form complicates model creation.}
{Monolingual model form need to be studied.}
Data preparation stage of all the libraries have high difficulty as presented in the previous section making it the second most difficult stage in the ML pipeline. 
\findings{Most libraries have problems in data cleaning.}{ Data cleaning 
	needs verification tools to ensure that all required steps in the process are performed. 
	%Unpopular data format can lead to more difficulty in cleaning like \weka. Which indicates design choice of data format can be a barrier.
}

Some of the libraries like \ho, \torch, \weka have comparatively higher percentage of posts making it equally difficult to model creation. 
\findings{\ho, \torch and \weka have 35.29\%, 22.95\% and 20.51\% 
	of posts, respectively, about data adaptation.}{The tradeoff in the design of data preparation APIs,e.g. use of custom formats, needs more study.}
% 	across these libraries 
% need deeper study and analysis. Specialized format like \weka's ARFF may 
% not be a good design decision.}


\textbf{RQ2:} Which  problems are more specific to library and which are inherent to ML? \newline


\findings{Type mismatches appear in most ML libraries.}{Type checkers are 
	desirable for ML libraries.}

\findings{Shape mismatch problems appear in higher percentage in deep 
	learning libraries. \keras is an outlier in this sub category with 5.5\% of 
	posts.}{Tool support for verifying shape and dimension compatibility
	is needed for deep learning libraries. Dependency of data on 
	model architecture needs to be verified and dynamic modification of the 
	network as per data shape may be needed.}

\findings{
	%\tensor, \keras, \mllib, \ho have higher percentage of runtime 
	%error during training with 5.32\%, 5.50\%, 5.88\% and 5.88\% respectively.
	Questions on exceptions/errors are prevalent.
}{
	Deep learning and distributed ML libraries show more error at training time. 
	This indicates static and dynamic analysis tools are needed for such 
	libraries.}

\findings{
	Parameter selection can be difficult.
}{
	Meta-heuristic strategies can be helpful.}

\findings{Choice of loss function is more problematic in deep learning libraries.}
{This indicates the necessity to develop automatic suggestion algorithms and tools 
	for selecting function for deep learning.}

\findings{\scikit and \caffe have higher percentage of questions about 
	training time accuracy and convergence (3.62\% and 3.78\% respectively).}{This 
	indicates the necessity to embed dynamic analysis of learning behavior along 
	with abstract APIs and the development of these analysis tools.}

\findings{\weka,~\ho,~\scikit,~\mllib form a strong correlated group with correlation coefficient greater than 0.84 between the pairs.}
{Analysis framework for one library can be reused in other library in this group.}


\findings{Deep learning libraries \torch,~\keras,~\theano~and~\tensor form another group with strong correlation of more than 0.86 between the pairs}{Problems of deep learning libraries currently follow a common pattern which can be leveraged by developing analysis framework for one library and studying how much solution is transferable from one library to another library.}


\textbf{RQ3:} Which libraries face problems in specific stages and which ones face difficulties in all stages?

\findings{\scikit has the highest number of posts on feature selection/extraction 
	subcategory (9.34\%).}{Blackbox abstraction for feature selection/extraction 
	APIs may not be suitable for ML libraries.} 

\findings{\scikit has abnormally high percentage of questions about model 
	creation compared to other libraries due to its lack of guidelines for model 
	selection.}{Recommendation support would be helpful in selecting models.
	%Abstract model selection APIs in \scikit didn't reduce the 
	%difficulties in model creation and model selection. Which gives intuition 
	%about an ML oriented abstraction for designing model creation and model 
	%selection APIs.
}

\findings{\scikit has more difficulty in hyper parameter tuning compared to 
	other libraries}{Due to the presence of a lot of optional parameters in the 
	APIs, the tuning of these parameters is more problematic than other libraries. 
	This gives intuition of having tools to suggest parameters that may have 
	effect on a particular model and particular problem. }


==> background.tex <==
\section{Background}
\label{sec:background}

We have selected the following 10 popular ML libraries for our study. 
Some of these libraries are specialized for deep learning.

\textbf{\tensor} \cite{abadi2016tensorflow} is an open source and popular
library. It was developed by engineers in Google Brain Team. This library uses
data flow graphs for doing computation. The nodes in the graph represent
operations to be done at that node and the edges in the graph represent the
tensors that flow from one node to another. This library originally developed
for doing research in Google's machine intelligence research organization
quickly gained popularly and helped development of other libraries built using
\tensor as backend also.

\textbf{\scikit} \cite{pedregosa2011scikit} is a popular machine learning
library used by machine learning engineers and data scientists. The library is
written using python programming language. It uses either \tensor or \theano
as the back end for doing internal computation. This library provides a rich set
of abstract APIs \cite{sklearn_api} to hide complex machine learning codes from
the user and make machine learning practice widely accessible to common people.

\textbf{\keras} \cite{chollet2015keras} is a popular deep learning library used
by python programmers. It provides high level abstract APIs to build neural
network and aims at using deep learning easier. Different components can be
connected one after another to form neural network without writing a whole bunch
of complex codes. \keras can run on top of \tensor or \theano back end to
perform internal computation needed. And those computations are hidden from the
users to lower the complexity barrier.

\textbf{\ho} \cite{candel2016deep} is a popular library that can work with
languages R, Python or Scala. It also has interface to Java programming
language. The library is specialized for doing deep learning tasks along with
normal machine learning and statistical modeling. The provide a work-flow like
system to build model called H2OFlow.It aims at covering Big data scale modeling
and predicting.

\textbf{Apache Spark \mllib}  \cite{meng2016mllib} is a subproject in spark to
provide machine learning support. It was originally developed at AMPLab,
University of California at Berkley. Then it was adapted by spark to further
develop and provide machine learning support with Spark since Spark version 0.8.
This library is aimed at doing fast, scalable and parallel machine learning in
spark cluster. Programs can be written in Scala or Python language and the spark
can run it on large scale cluster data.

\textbf{Apache \mahout} is project  by Apache Software Foundation. It provides
large scale machine learning support in cluster. This is specialized library
from collaborative filtering, classification and clustering related tasks. It is
provided as a Scala DSL with support to distributed linear algebra computation
that helps quickly building models to large scale. 

\textbf{\weka} \cite{holmes1994weka} is Java based machine learning library.  It contains
machine learning algorithms specialized for data mining tasks. It provides API
support for data preparation, classification, regression, clustering and
association rules mining tasks. \weka also provides a GUI to help creating the
model easier.

\textbf{\caffe} \cite{jia2014caffe} is deep learning library developed by Berkley
AI Reasearch (BAIR). Models and Optimizations are defined in configuration file
in \caffe. Speed and performance makes \caffe a popular library to researchers.
Main coding environment for \caffe is C++ but a version for python language
called pycaffe is also used by the users.

\textbf{\torch} \cite{collobert2002torch} is a GPU first library where a fast
scripting language LuaJIT is used for writing codes. It also provides a support
to C/CUDA implementation of models. %is a scientific computing framework with
% wide support for machine learning algorithms that puts GPUs first. It is easy
% to use and efficient, thanks to an easy and fast scripting language, LuaJIT,
% and an underlying C/CUDA implementation.
%A summary of core features are :a powerful N-dimensional array,lots of routines
% for indexing, slicing, transposing,amazing interface to C, via LuaJIT,linear
% algebra routines,neural network, and energy-based models,
%numeric optimization routines,Fast and efficient GPU support,
%Embeddable, with ports to iOS and Android backends.
\textbf{\theano} \cite{bergstra2011theano}
is a python library that helps to create models using multi dimensional array.
It uses GPU to provide faster computing, provides some self verification and
unit testing to diagnose many types of errors made at runtime.









==> chosemodel.tex <==
\begin{figure}[t]
	\includegraphics[width=\columnwidth]{chosemodel}
	\caption{A Stack Overflow question on choice of model stage by using a library}
	\label{fig:chosemodel}
\end{figure}

==> dataprep.tex <==
\begin{figure}[t]
	\includegraphics[width=\columnwidth]{dataprep}
	\caption{An example question on data preparation stage}
	\label{fig:dataprep}
\end{figure}

==> datasetfull.tex <==
\begin{table*}[ht]
\caption{Data of different machine learning frameworks}
\begin{tabular}{\textwidth}{ |l|r|r|r|r|r|r|r|r|r|r|r| } 
 \hline
 ML Library  & Score $\ge$ 0  & Score $\ge$ 1 & Score $\ge$ 2 & Score $\ge$ 3 & Score $\ge$ 4 & Score $\ge$ 5 & Score $\ge$ 6 & Score $\ge$ 7  & Score $\ge$ 8 & Score $\ge$ 9 & Score $\ge$ 10 \\ 
 \hline
 \mllib \cite{meng2016mllib} & 1688 & 929 & 498 & 272 & 173 & 123 & 91 & 66 & 51 & 43 & 38 \\ 
 \hline
 \caffe \cite{jia2014caffe}& 2339 & 1320 & 620 & 318 & 192 & 135 & 104 & 79 & 63 & 50 & 46 \\ 
 \hline
 \weka \cite{holmes1994weka}& 2512 & 1216 & 568 & 293 & 181 & 127 & 89 & 62 & 40 & 34 & 26 \\ 
 \hline
 \ho \cite{candel2016deep} & 771 & 452 & 167 & 73 & 34 & 20 & 14 & 10 & 5 & 4 & 4 \\ 
 \hline
 Scikit learn \cite{pedregosa2011scikit}& 9246 & 5302 & 2898 & 1759 & 1188 & 849 & 616 & 478 & 387 & 328 & 268 \\ 
 \hline
 \tensor\cite{abadi2016tensorflow} & 2115 & 10109 & 4962 & 2769 & 1827 & 1318 & 1003 & 802 & 656 & 535 & 458 \\ 
 \hline
 \theano \cite{bergstra2011theano} & 2332 & 1341 & 711 & 421 & 265 & 198 & 142 & 99 & 76 & 59 & 46 \\ 
 \hline
 \torch \cite{collobert2002torch} & 1226 & 640 & 312 & 161 & 91 & 61 & 49 & 31 & 25 & 23 & 17 \\ 
 \hline
 \keras \cite{chollet2015keras} & 5708 & 3323 & 1751 & 953 & 568 & 385 & 287 & 216 &  170 & 134 & 99 \\ 
 \hline
 Apache \mahout & 1186 & 610 & 293 & 160 & 103 & 64 & 45 & 32 & 27 & 23 & 21 \\ 
 \hline
 Total & 49903 & 26103 & 13172 & 7376 & 4735 & 3353 & 2497 & 1918 & 1533 & 1257 & 1045 \\ 
 \hline
\end{tabular}
\end{table*}

==> discussion.tex <==
\section{Discussion of Results}
TBD whether needed. 


==> evalaution.tex <==
\begin{figure}[t]
	\includegraphics[width=\columnwidth]{evaluation}
	\caption{A stackoverflow question on evaluation phase of using a library}
	\label{fig:evaluation}
\end{figure}

==> evaluation.tex <==
%\input{intracharts}
%\input{intratable}
%\section{Analysis and Results}
%\label{sec:evaluation}

\section{Intra-Library Analysis}
\label{sec:intra-library}

%\input{interold}
In this section, we 
% discuss our study results on the problems raised in the \sof posts for each library individually.
%We 
discuss the potential strengths and weaknesses of each library 
w.r.t. our classification in \figref{fig:classes}.
% at different stages and (sub)categories. 
The statistics are shown in \tabref{tbl:cat} and \tabref{tbl:subcat}. 

\input{intranew}

\section{Inter-Library analysis}
\label{sec:inter-library}

%\input{librarycatchart} 

In this section, we  present our analysis and observations across ML libraries. 
%In the following section, we present the analysis results that focus on a single ML library at-a-time. 
%
% In this section we present the results of our observation of developer behaviors
% in using different machine learning frameworks \cite{stages}. We also classify
% the problems faced in each stage into different categories.
%
%
We study the strengths and weaknesses of different ML libraries 
in terms of each of the top-level categories defined in \figref{fig:classes}.
% We study different libraries and see the strong and weak part of 
% different libraries at different stages of machine learning in terms 
% of developers difficulty. 
% The distributions of the percentages of questions over stages of all 
% libraries are shown in the heatmap in \tabref{tbl:cat} and \tabref{tbl:subcat}.
The distribution of questions over stages of all 
libraries are shown in \tabref{tbl:cat} and \tabref{tbl:subcat}.

%\figref{fig:interlib}. 

%\input{interlibanalysis}

\input{internew}

\input{misuses}

\input{inter-group}



==> future.tex <==
\section{Future Works}
We observe from our study that the machine learning library can be improved with software design best practices that can. We want to study how the machine learning libraries can be modularized by following standard software design principles \cite{parnas1972criteria}. We also want to explore whether viewing machine learning from programming language design using probabilistic programming approaches can overcome a lot of these issues \cite{prekopa2003probabilistic,ppaml}. Static analysis and debugging in machine learning libraries is also an interesting thing that we want to study. 

==> hyperparam.tex <==
\begin{figure}[t]
	\includegraphics[width=\columnwidth]{hyperparameter}
	\caption{A stackoverflow question on hyper parameter tuning phase of using a library}
	\label{fig:hyper}
\end{figure}

==> inter-data.tex <==
\subsubsection{Data Preparation}

%We study the subcategories of data preparation in this section. 


\textbf{Data adaptation}

As shown in \tabref{tbl:subcat}, the percentages of questions about data 
adaptation across libraries have SD of 8.70\% and IQR of 12.93\% which 
indicates a considerable variation across the libraries. We also see that the 
libraries like \ho, \torch and \weka have respectively 35.29\%, 22.95\% and 20.51\% 
of questions related to using library APIs to adapt data to pipelines. %
%From our outlier table we see no libraries are outlier as per definition of outlier. 
That shows significant difficulties and would call for research effort to improve this stage.
%But still \weka, \torch and \ho have the larger volume of questions related 
%to data preparation indicating data adaptation from data source to machine 
%learning pipeline is needs research for improvement. 
We also see questions about \weka's custom data format 
to which developers are not familiar. 
This leads us to the first finding and implication.
%This leads us to the observation that if a library uses unfamiliar data 
%format or if the conversion gap from raw data to pipeline data is more then 
%adapting data becomes a problem for that library. 

%\findings{\ho, \torch and \weka have 35.29\%, 22.95\% and 20.51\% 
%of posts, respectively, about data adaptation.}{The tradeoff in the design of data preparation APIs,e.g. use of custom formats, needs more study.}
% 	across these libraries 
% need deeper study and analysis. Specialized format like \weka's ARFF may 
% not be a good design decision.}
\textbf{Featuring}

From \tabref{tbl:subcat}, percentages of questions related to feature 
extraction/selection has SD of 3.03\%, median of 0.92\% and IQR of 4.17\%. 
Among the libraries, users of \scikit have the most questions of 9.34\% even 
though this library has APIs for auto-selecting features. 
%But we observe the percentage of questions about feature extraction/data 
%preparation in \scikit is more than mean +2SD. 
%This could suggest that developers using this library face more difficulty on 
%feature extraction/selection compared to other libraries. 
\ho, \weka and \mllib follow with 5.88\%, 4.27\% and 4.20\%, 
respectively. This suggests that existing feature extraction/selection 
support might not yet be sufficient to ease the ML practice. 
Surprisingly, \tensor users have comparatively fewer difficulties in data 
preparation, especially in feature engineering. 
%There are some difficulties in adapting TFRecords (a data format used by \tensor) or storing data in this format. 
The reason could be attributed to multiple adapters \tensor provides to read and 
store dataset. The dataset is stored as elements with the same size and 
each element can contain one or more Tensor objects. Each Tensor object also 
has type and shape information added to it. Using Tensor objects 
and providing functionality to read raw data and forming dataset using 
Tensor objects reduces adaptation and data cleaning related errors. 
% COMMENT-HR: following is too much detail.
%An example of 
%how the dataset is represented as a tensor from a random uniform matrix of 4*
%10 size is given in the following code snippet:
%
%\input{tensor}
%
%We see that the dataset is read and parsed as tensor by the library with type and shape information. 
%The library enables easier adaptation of data as well as debugging any dataset related problem by tensor debug. 

%\findings{\scikit has the highest number of posts on feature selection/extraction 
%subcategory (9.34\%).}{Blackbox abstraction for feature selection/extraction 
%APIs may not be suitable for ML libraries.} 

%	A new way of ML oriented abstraction may be needed while engineering 
%  feature selection/extraction APIs in ML libraries. }

\textbf{Type mismatch}

Type mismatch questions have median of 1.61\%, SD of 1.02\%, and IQR of 1.80\%. 
The smaller IQR indicates that type mismatch appears in most of the 
libraries. \scikit, \mllib, \theano and \tensor  have higher difficulties in 
type-related problems with 2.92\%, 2.52\%, 2.08\% and 2.02\%, respectively. 
\mllib uses a custom data format called RDD that seems to make type-related 
problems more common to this library. There are also questions about failures 
due to type mismatch in \scikit, \tensor and \theano as their APIs have type 
requirements that are not currently checked. A static analysis tool might be 
able to prevent the majority of these problems.  
\findings{Type mismatches appear in most ML libraries.}{Type checkers are 
	desirable for ML libraries.}
Finding 5 provides the indication that in machine learning libraries type checking and ML specific type system engineering is not being done properly. So type checkers are 
desirable for ML libraries
% This problem starts passing from the data preparation stage and 
% create fatal error stopping the training.
% The training fails due to this type mismatch problem. 
% COMMENTS-HR: don't know what above is trying to say. Doesn't seem to add anything.
% \input{type}
% For example Figure \ref{fig:type} shows a question on type mismatch. 
% The whole training process failed in the middle where the library found an unwanted type.
% COMMENTS-HR: I think this is an easy one to elide, as type mismatch 
% is well understood issue.

%\findings{Type mismatches appear in most ML libraries.}{Type checkers are 
%desirable for ML libraries.}

\textbf{Shape mismatch}

Shape mismatch related questions have median of 0.75\%, SD of 1.70\%, and IQR 
of 2.03\%. This problem appears in all deep learning library in which \keras 
is an outlier with 5.50\%. In these libraries, shapes of neurons at adjacent 
layers must be compatible otherwise the library will throw exceptions during 
training or fail during prediction. 
Such a problem is shown in \figref{fig:shape}.

 \findings{Shape mismatch problems appear in higher percentage in deep 
 	learning libraries. \keras is an outlier in this sub category with 5.5\% of 
 	posts.}{Tool support for verifying shape and dimension compatibility
 	is needed for deep learning libraries. Dependency of data on 
 	model architecture needs to be verified and dynamic modification of the 
 	network as per data shape may be needed.}
 As pointed out in Finding 6, tool support for verifying shape and dimension compatibility
 is needed for deep learning libraries. Dependency of data on 
 model architecture needs to be verified and dynamic modification of the 
 network as per data shape may be needed
 \input{shape}

Abstract APIs that hide the details of inner-working of the deep networks can 
further complicate matters. 
To illustrate consider the following \keras code.

\input{kerasstatic} 

The error is at line 6 where an invalid value of $(31,3)$ is passed 
to $input\_shape$. The accepted answer suggests that $input\_shape$ should be 
$(32,1)$ instead. The user could not verify statically whether the built 
network is matching in shape or there is any unconnected or extra port while 
building the model. If we had the tools that could tell the developer 
that using dimension (32,1) can cause 2 out of 3 ports of the next layer to 
be unconnected then it would be much easier for the developer to find these 
errors by themselves. This kind of errors could be detected by program analysis 
and by providing feedback to the users. In fact, many discussions in these 
high-scored posts call for richer analysis features.

%For example, see \figref{fig:shape} that has a sample question on shape
%mismatch.
%Due to highly abstract APIs in \keras users don't have a lot of information outside the box about what is happening behind the seen and creates runtime failure unexpectedly. This indicates that, abstraction in machine learning and deep learning libraries can be an useful direction of research. 
%Static and dynamic analysis (or even more capable typechecking) can resolve a
%lot of issues related to shape mismatch, type mismatch, and others. But current
%libraries lack any verification features. 

%\tensor and \theano take a good share of shape related problems having 
%respectively 2.62\%  and 2.083\%. \scikit follows them with 1.87\%. \scikit 
%is also a highly abstract API based library hiding all the machine learning 
%magic from the developer. So we see deep learning libraries like \keras, 
%\tensor, \theano have more shape related problem and shape related problems 
%also appear due to higher abstraction.  

%\findings{Shape mismatch problems appear in higher percentage in deep 
%learning libraries. \keras is an outlier in this sub category with 5.5\% of 
%posts.}{Tool support for verifying shape and dimension compatibility
%is needed for deep learning libraries. Dependency of data on 
%model architecture needs to be verified and dynamic modification of the 
%network as per data shape may be needed.}

\textbf{Data Cleaning}

As shown in \tabref{tbl:subcat}, data cleaning related questions across the 
libraries have median of 1.82\%, SD of 1.22\% and IQR of 1.61\%. Most of the 
libraries have questions about data cleaning stage except for \ho and \torch. 
In fact, this is obviously needed step in any data science pipelines. 
Libraries \scikit, \weka and \mllib have the most questions with 3.62\%, 3.42\% %
and 2.52\%, respectively. The abstract APIs in these libraries sometimes make 
cleaning fail. For example, the \code{nan} values in the \code{dataframe} 
needs to be converted first into numpy \code{nan} type before they can be 
cleaned using APIs provided by \scikit. 
Furthermore, these failures do not clearly indicate the root cause
making diagnostics difficult.
\findings{Most libraries have problems in data cleaning.}{ Data cleaning 
	needs verification tools to ensure that all required steps in the process are performed. 
	%Unpopular data format can lead to more difficulty in cleaning like \weka. Which indicates design choice of data format can be a barrier.
}
Finding 7 shows that data wrangling or data cleaning is an important part of data preparation which needs tooling support. 
% When the failure happens, the user 
% does not have any clue what causes it. %
% %These type of problems also indicate necessity of static analysis and dynamic 
% %analysis tools for machine learning. 

%\findings{Most libraries have problems in data cleaning.}{ Data cleaning 
%needs verification tools to ensure that all required steps in the process are performed. 
%Unpopular data format can lead to more difficulty in cleaning like \weka. Which indicates design choice of data format can be a barrier.
%}


%\paragraph*{\textbf{Libraries that use uncommon or new formats of 
%		data create difficulties in data preparation.}}

%We can observe in \figref{fig:interlib} that the developers using
%\weka and \mllib library face more difficulty in the data preparation 
%stage while adapting data to the ML Library. 
%For \weka 36/127 questions and for \mllib 41/123 focused on data 
%preparation issues.
%\input{ob1}
%As we observe in a sample question in Figure \ref{fig:ob1weka} that the user is
%trying to use a dataset from a well-known ML dataset repository \cite{uci}. 
%Usually these datasets are preprocessed to do machine learning and
%importing these datasets can be done directly. But an user of \weka user is not
%able to successfully adapt the dataset to the library for training due to the
%failure of conversion to ARFF format needed by the library. 
%Similarly, developers using Apache Spark \mllib also have a higher percentage of difficulties
%during the data preparation stage because it uses RDD format of data
%which is a less popular format. Adapting the data for the library,
%converting from popular data formats to the format required or preferred by the
%library are some common problems faced by the users when the library uses less
%popular data formats. 

%\paragraph*{\textbf{\tensor users face less difficulty in data 
%		preparation stage due to tensor usage}}
%Surprisingly, \tensor has comparatively fewer difficulties in data preparation. There are some difficulties in adaptation TFRecords (a data format used by \tensor) or storing data in this format. 
%This could be because this ML library provides multiple adapters 
%to read and store data.
%In \tensor, the dataset is stored as elements of same size and each element can contain one or more Tensor objects. 
%Each Tensor object also has type information and shape information added to it. 
%Using Tensor objects and providing functionalities to read raw data and forming dataset using Tensor objects reduces errors, adaptation and data cleaning related problems. 
%An example of how the dataset is represented as a tensor from a random uniform matrix of 4*10 size is given in the following code snippet:
%\input{tensor}
%We see that the dataset is read and parsed as tensor by the library with type and shape information. 
%The library enables easier adaptation of data as well as debugging any dataset related problem by tensor debug. 
%\torch and \theano also use tensors as their data structure. 
%Although they have comparatively few problems in the data preparation stage, the data adaptation and loading APIs create slightly more difficulties compared to \tensor in these libraries. 
%For \tensor 234/1318 questions were about data preparation that is proportionally lower compared to other libraries.


==> inter-eval.tex <==
\subsubsection{Evaluation of models}

This category has median of 6.0\%, SD of 2.9\% and IQR of 4.8\%. %
%We see from our study that the developers have from 1\%--10\% of questions 
% about this stage. 
The visualization and output interpretation subcategories do not have
enough data to make meaningful interpretations.

\textbf{Evaluation Strategy}

Selection of evaluation strategy has median of 1.86\%, SD of 2.64\% and 
IQR of 3.86\%. This indicates that this functionality varies more across different 
libraries. \weka, \tensor and \mllib have more questions on evaluation strategy 
using the APIs having 8.54\%, 5.24\% and 5.04\%, respectively. 
We believe that this might be because these three libraries provide a 
rich set of features for this task.

==> inter-group.tex <==
\subsubsection{Grouping Libraries} 

We studied the libraries to see if there is some similarity of patterns among the libraries compared by the distribution of problems at different stages. 

\input{correlationoflibs}

From the chart in \figref{fig:corrlib}, we group the libraries into the following categories:

\textbf{Group 1.\ }  \weka,~\ho,~\scikit,~and~\mllib form a strongly correlated group with correlation coefficient greater than 0.84 between the pairs. Other than \ho, other libraries in this category are not used for deep learning. This suggests that the problems appearing in these libraries have some correlation and the difficulties of one library can be described by the difficulty of other libraries in the group.

\findings{\weka,~\ho,~\scikit,~\mllib form a strong correlated group with correlation coefficient greater than 0.84 between the pairs.}
{Analysis framework for one library can be reused in other library in this group.}
Finding 13 suggest, analysis framework for one library can be reused in other library in this group.

\textbf{Group 2.\ } \torch,~\keras,~\theano,~and~\tensor form another group with strong correlation of more than 0.86 between the pairs. These libraries are specialized for deep learning. This suggests that deep study of one library can also be useful in the analysis for other deep learning libraries. It means that the problems are cross related to the libraries for this category. 
\findings{Deep learning libraries \torch,~\keras,~\theano~and~\tensor form another group with strong correlation of more than 0.86 between the pairs}{Problems of deep learning libraries currently follow a common pattern which can be leveraged by developing analysis framework for one library and studying how much solution is transferable from one library to another library.}
Finding 14 suggests problems of deep learning libraries currently follow a common pattern which can be leveraged by developing analysis framework for one library and studying how much solution is transferable from one library to another library.

==> inter-model.tex <==
\subsubsection{Modeling}

This category has the most questions in our study with median of 27\%.
%The libraries we studied have around 25\%--45\% of questions about using the 
%libraries at modeling stage. 
We now present observations about its subcategories.
% Observations about its subcategories are presented in the following subsections. 

\textbf{Model creation}

As shown in \tabref{tbl:subcat}, questions about model creation has median of 
23.22\%, SD of 6.70\% and IQR of 3.53\% which indicates that all 
libraries have major problems in this step. \mahout is an outlier with almost 
half number of questions about this. Since \mahout is used for ML on clusters, 
this could be attributed to the difficulty in creating 
models on clusters or doing distributed ML. 
%
%Similar is the case with \mllib which is also used to do parallel machine 
%learning in cluster. Though \mllib is not an outlier, it still has 23.52\% of 
%posts about model creation.

\input{mahout}

%\mllib and \mahout (These libraries specialized for distributed machine learning)
 %users face higher difficulties in model creation, running model in parallel 
%following map-reduce paradigm, selecting the appropriate model. 
%
\figref{fig:mahout} shows an example question asking about creating a MapReduce version of a model in \mahout.

Deep learning libraries like \caffe, \keras, \theano and \tensor also have 
higher percentages of questions about model creation with 26.52\%, 25.88\%, 23.43\% and 23.01\%, respectively. This shows that model creation 
for deep neural networks is difficult as well. 
 
%\findings{Model creation is the most challenging (yet critical) in ML 
%pipeline, especially for libraries supporting distributed ML on 
%clusters like \mahout and \mllib. 
%with 43.75\% and 23.52\% questions, respectively. 
%\mahout is an outlier in this step. 
%}{This calls for tool support in creating models, 
%especially in distributed machine learning.} 

%\findings{Deep learning libraries \caffe, \tensor, \keras and \theano have 
%respectively 26.51\%, 23\%, 26.17\%, 23.44\% posts about model creation. }{
%Like parallel machine learning model creation in deep learning libraries is 
%also difficult. It can be of substantial help if some architecture 
%verification tool and autonomous model creation support is provided by deep 
%learning libraries.}
 
When we study the questions about \caffe we see that \caffe users have 
problems in model creation due to the  dependency of the model on multiple 
files. To create a model successfully, one  needs to make a schema file in 
protobuf format, create a solver file and write code in C++ or Python to 
build the model~\cite{caffetutorail}. 
Having several components complicates matters.
% For example, this tutorial describes multiple components in separate files 
% needed to build a model successfully using \caffe and Python. 
% This gives us some intuition that the framework 
% where the model depends on multiple components or there are more than one way 
% to create the same model introduces technical challenges in the model 
% creation phase. 
% \caffe is mainly used for deep learning and was developed by Berkley Vision. 
% \caffe models are defined in a plain text protocol buffer schema (prototxt), 
% which increases the complexity of using this library to many users. A lot of 
% questions on \caffe in \sof are about creating the schema in the prototxt 
% file and failures of models defined using prototxt files. 
In our study, 36 out of 135 questions about \caffe are about model creation problems. 
% This gives us indication that model creation can be complicated 
% if the operation depends on multiple files or modules.

% \findings{Plain text representation of models could add complications to 
% model creation.}{More intuitive representation designs of models, such as graphs 
% in \tensor, would help and need to be studied.}  

%\findings{Multilingual form complicates model creation.}
%{Monolingual model form need to be studied.}

\textbf{Model selection}

This subcategory has fewer questions than others with median of 0\%. 
%Model selection subcategory have the mean of 0.40, SD of 0.64 and IQR of 0.587. 
\scikit is an outlier with 2.10\%. While \scikit APIs abstracts the details 
of underlying ML algorithms, it does not provide enough guidelines on which 
model would be the best for given data. 
%This suggests the need to develop recommendation systems to address this need.

%\findings{\scikit has abnormally high percentage of questions about model 
%creation compared to other libraries due to its lack of guidelines for model 
%selection.}{Recommendation support would be helpful in selecting models.
%Abstract model selection APIs in \scikit didn't reduce the 
%difficulties in model creation and model selection. Which gives intuition 
%about an ML oriented abstraction for designing model creation and model 
%selection APIs.
%}

\textbf{Model conversion}

Converting models trained using one library and using it with another library 
is a common problem. 
%For example, let's consider someone has trained an SVM 
%model on a particular dataset D. The user then wants to load the model in 
%\weka and use that for future prediction. 
Some libraries provide support to convert model for use with other libraries 
but such support is not always adequate. The developers often have questions 
about reusing trained models in other platforms. Percentages of question in 
this subcategory have median of 1.54\%, SD of 1.71\% and IQR of 2.97\%. %
\torch, \caffe, \weka lead this subcategory with 4.91\%, 3.79\% and 3.41\%, 
respectively. This suggests that interoperability of models across libraries 
is needed.

\textbf{Model Load/Store}

Loading/Storing model has mean of 2.54, SD of 1.87 and IQR of 2.62 across the 
libraries. \ho and \mllib leads this category with 5.88\% and 5.02\% 
respectively. 


==> inter-predict.tex <==
\subsubsection{Prediction}

\textbf{Prediction Accuracy}

Questions about prediction accuracy across the libraries have median of 4.60\%, SD of 2.44\% and IQR of 3.30\%. %
Libraries with abstract APIs like \weka, \keras, \caffe, \scikit and \mllib have the highest volume of questions with 8.54\%, 6.81\%, 6.10\%, 5.25\% and 5.04\%, respectively. 
%This indicates that libraries with high abstraction like \scikit, \keras, \weka have more problems in prediction stage.  
Though \caffe has fewer questions in model creation, it has higher difficulties in prediction stage.

\textbf{Model reuse}
This subcategory has median of 0\%, SD of 0.60\% and IQR of 0.23\%.
\keras and \weka are outliers with 1.37\% and 1.71\% of questions about 
model reuse.

\textbf{Robustness}
This subcategory has median of 0.15\%, SD of 0.59\%, and IQR of 0.85\%.

For both model reuse and robustness subcategories, developers are just 
becoming aware of the possibility and seeking clarifications about it.


==> inter-train.tex <==
\subsubsection{Training}
%
%In our study we have found that, across libraries on average 18\% questions, 
%were about training. The study of questions at this stage reveals following 
%findings. 

We now present observations about the training category that 
has on average 18\% questions across libraries.

\textbf{Error/Exception}

Error/Exception subcategory has the median of 5.10\%, SD of 1.80\% and IQR of 2.71\%. 
All the libraries have issues on runtime error/exception. 
Surprisingly, though model creation seems problematic in \caffe, 
runtime failure is very low in \caffe with 0.76\%. 
\mllib, \ho, \keras, \tensor and \scikit have higher percentage of runtime errors with 5.88\% and 5.88\%, 5.50\%, 5.32\% and 4.78\%, respectively.
This suggests that debugging and 
monitoring facilities for ML needs much improvement
to help developers resolve error/exception independently.

\findings{
	%\tensor, \keras, \mllib, \ho have higher percentage of runtime 
	%error during training with 5.32\%, 5.50\%, 5.88\% and 5.88\% respectively.
	Questions on exceptions/errors are prevalent.
}{
	Deep learning and distributed ML libraries show more error at training time. 
	This indicates static and dynamic analysis tools are needed for such 
	libraries.}

We see in Finding 8 deep learning and distributed ML libraries show more error at training time. 
This indicates static and dynamic analysis tools are needed for such 
libraries.
We have observed that the lack of rich and interactive debugging tools makes 
building ML models difficult. 
A number of problems faced by developers, e.g. when a model 
is throwing an exception at training time, a model is not converging or 
learning as the iteration of training goes on, a model is not predicting 
well, 
% model creation is not correct and producing incorrect results, 
% a model is not performing well for a particular instance of a problem, 
etc, can be 
minimized to a great extent with effective debugging tools. Fortunately, some 
recent work has started to address these issues~\cite{chakarov2016debugging,tdebug}, 
but much more work is needed. Due to the lack of debugging 
tools to monitor pipelines causes of failure are hard to identify. 
More abstract deep learning libraries 
throw more runtime exception during training, e.g. see Figure \ref{fig:ob6}.

\input{keraserr}

% COMMENT-HR: A lot of this discussion is redundant.
%For example in Figure \ref{fig:ob6} a \keras (An abstract library on top of 
%\tensor or \theano backend) developer has built the model successfully yet 
%they get an error at runtime. The reason is that model building in deep 
%learning model needs to successfully connect multiple hidden layers along 
%with the input and output layer. But with abstract libraries, the user 
%doesn't have any tools to inspect within the model. Furthermore, while 
%connecting these APIs to build the neural network the user has many places of 
%single point failure starting from dimension mismatch, wrong activation 
%function usage as well creating hidden loops with a performance overhead. 
%20 out of 385 questions for \keras are about training time error 
%%
%We have found 20 questions related to training time error out of 385 
%questions in \keras. 

\textbf{Parameter selection}

Questions about parameter selection have median of 4.50\%, SD of 2.60\% and 
IQR of 2.89\%. This shows a wide variation between libraries.
%From this statistics we seen the deviation around mean is large and libraries 
\caffe and \torch have comparatively more problems with 9.10\% and 8.20\%, 
respectively. Libraries like \keras , \weka, \ho, \mllib shows larger 
percentage of questions on choice of parameters. 

\findings{
	Parameter selection can be difficult.
}{
	Meta-heuristic strategies can be helpful.}
For selecting parameter meta-heuristic strategies can be helpful.

\textbf{Loss function}

Choice of Loss function has the median of 2.16\%, SD of 1.86\% and IQR of 2.62\%. %
This shows that the loss function choice varies across the libraries. %
All deep learning libraries like \caffe, \keras, \tensor and \torch have the 
highest percentages of 6.10\%, 4.09\%, 3.74\% and 3.30\%, respectively. %
This indicates necessity of further research on the usage of loss function in 
deep learning libraries. 

\findings{Choice of loss function is more problematic in deep learning libraries.}
{This indicates the necessity to develop automatic suggestion algorithms and tools 
	for selecting function for deep learning.}

Finding 10 gives us evidence to say is is necessary to develop automatic suggestion algorithms and tools 
for selecting function for deep learning.
% COMMENT-HR: Can make the implication above shorter, if space needed.

\textbf{Optimizer}

Optimizer subcategory has median of 1.07\%, SD of 1.07\% and IQR of 1.46\% across libraries. %
\torch, \tensor, \caffe have respectively 3.30\%, 2.77\% and 2.30\% of 
questions about optimizer which is higher compared to other libraries. This 
suggests that choice of optimizer is more relevant for the deep learning 
libraries. 

\textbf{Performance}

This subcategory has median of 3.20\%, SD of 1.80\% and IQR of 2.87\%. %
We see that the distributed ML and deep learning libraries like \keras, \ho, \mllib 
and \tensor, have higher percentage of questions related to performance 
having 6.27\%, 5.88\%, 5.04\% and 4.87\%, respectively. Performance related 
problems here appear due to runtime, memory usage and convergence. 

\textbf{Training accuracy}

%Training time accuracy with the progress of training related questions fall 
%into this sub category. 
This subcategory has fewer questions than others with median of 0.97\%. %
\caffe and \scikit have the highest share with 3.78\% and 3.62\%, 
respectively. \scikit is a library with highly abstract APIs and large number 
of optional parameters to be selected. Due to the abstraction, the impact 
of parameter values on training accuracy could be unclear to developers.
% This gives intuition that, in machine 
% learning libraries abstracting away everything may not be the right solution 
% and a new form of ml oriented abstraction may be needed. 

\findings{\scikit and \caffe have higher percentage of questions about 
training time accuracy and convergence (3.62\% and 3.78\% respectively).}{This 
indicates the necessity to embed dynamic analysis of learning behavior along 
with abstract APIs and the development of these analysis tools.}

Finding 11 indicates the necessity to embed dynamic analysis of learning behavior along 
with abstract APIs and the development of these analysis tools.


==> inter-tune.tex <==
\subsubsection{Tuning}
This category involves questions about selection of hyper parameters
and tuning strategies. 

\textbf{Tuning strategy selection}
This subcategory has median of 0.60\%, SD of 1.82\% and 
IQR of 1.45\% suggesting a variation.
\ho is an outline in this subcategory having 5.88\% questions.
We believe \ho APIs for tuning strategy selection are newer
and need improvement.

\textbf{Tuning paramater selection}
This subcategory has median of 0, SD of 0.24, and IQR of 0 
because not too many libraries have questions about it.
\scikit and \tensor are the outliers in tuning parameter category. This was 
expected as \scikit has a lot of optional parameters to be selected and those 
parameters have effect on the convergence and accuracy.

\input{tune}

%Hyperparameter tuning stage involves selection of hyper parameters that need 
%to be tuned, tuning strategy selection etc. 
%
%\subsubsection{Hyperparameter selection}
%
%
%\scikit and \tensor are the outliers in tuning parameter category. This was 
%expected as \scikit has a lot of optional parameters to be selected and those 
%parameters have effect on the convergence and accuracy. We dont' want to make 
%a model complicated by unnecessary parameter tuning but want to tune the 
%right parameter to reach the maximum result. This gives us intuition that 
%providing the burden of selecting a lot of parameters via the API to the 
%programmer can be a cause of problem in hyper parameter tuning stage. 
As an example, consider the API below to create \texttt{AdaBoostClassifier} 
with 5 optional parameters initialized to some default values. 

\input{sklearn} 

The \texttt{base\_estimator} is set to \texttt{None} but the user may need to choose an 
estimator to get the best performance. Learning rate is by default set to 1.0. %
At this learning rate, it is highly likely that the model will not learn 
anything. So the user may often use these APIs incorrectly and wonder why ML 
model is not producing the useful result. Since these are optional 
parameters, the user will not even get any error or warning. Finding good 
values for these parameters and tuning them to make the best model, avoiding 
over-fitting are frequent questions among developers using \scikit. There 
have been some GitHub issues filed to the repository of \scikit as bugs (See 
\figref{fig:tune} for an example) but the underlying problem was that the 
developer was not able to trace why the model is not showing expected 
accuracy, and unable to tune hyperparameters. We have found 36 questions out 
of 849 in \scikit asking help about hyperparameter tuning.

\findings{\scikit has more difficulty in hyper parameter tuning compared to 
other libraries}{Due to the presence of a lot of optional parameters in the 
APIs, the tuning of these parameters is more problematic than other libraries. 
This gives intuition of having tools to suggest parameters that may have 
effect on a particular model and particular problem. }
From Finding 12 we see, due to the presence of a lot of optional parameters in the 
APIs, the tuning of these parameters is more problematic than other libraries. 
This gives intuition of having tools to suggest parameters that may have 
effect on a particular model and particular problem.


==> inter.tex <==
\paragraph{title}

==> interest.tex <==
%\begin{figure*}[t]
%	\centering
%	\begin{subfigure}[t]{0.48\textwidth}
%		 \centering
%		\includegraphics[width=\linewidth]{qvsyear}
%		\caption{Posts VS Year}
%	\end{subfigure} \hfill
%	\begin{subfigure}[t]{0.48\textwidth}
%		\centering
%		\includegraphics[width=\linewidth]{duvsyear}
%		\caption{Distinct USer VS Year}
%	\end{subfigure} \hfill
%	\caption{Growing interest}
%	\label{fig:interest}
%\end{figure*}
\begin{figure}[t]
	\includegraphics[width=\columnwidth]{mlpop}
	\caption{Growing interest of machine learning}
	\label{fig:interest}
\end{figure}

==> interlibanalysis.tex <==
\begin{figure}[t]
	\includegraphics[width=\columnwidth]{heatmap1}
	\vspace{-1.5em}
	\caption{Heatmap showing the percentage of questions asked for the top-level categories in \figref{fig:classes}.}
	\label{fig:interlib}
\end{figure}

==> internew.tex <==
\input{inter-data}

\input{inter-model}

\input{inter-train}

\input{inter-eval}

\input{inter-tune}

\input{inter-predict}








%\paragraph*{\textbf{Libraries that provide more optional parameters complicate hyperparameter tuning}}
%Hyperparameter tuning related questions are comparatively frequent among the
%\scikit users. Usually, \scikit APIs take a lot of optional parameters.
%For example, we see an API to create \texttt{AdaBoostClassifier} below with 5 optional
%parameters initialized to some default values. 
%\input{sklearn} 
%The best\_estimator is set to None but the user may need to choose an estimator to
%get the best performance. Learning rate is by default set to 1.0. At this
%learning rate, it is highly likely that the model will not learn anything. So the
%user may often use these APIs incorrectly and wonder why ML model is
%not producing the useful result. Since these are optional parameters, the user will not even get any error or warning. Finding good values for these parameters and tuning them to make the best model, avoiding over-fitting are frequent questions among developers using \scikit. There have been some 
%Github issues filed to the repository of \scikit as bugs 
%(See \figref{fig:tune} for an example)
%but the underlying problem was that the developer was not able to trace why the model is not showing expected accuracy, and unable to tune hyperparameters. We have found 36 questions out of 849 in \scikit asking help about hyperparameter tuning.





%\paragraph*{\textbf{More abstract deep learning libraries have more runtime error}}
%In \keras, a highly abstract deep learning library, developers get the comparatively higher error at runtime. 
%\input{keraserr}
%For example in Figure \ref{fig:ob6} a developer has built the model successfully
%yet they get an error at runtime. The reason is that model building in deep
%learning model needs to successfully connect multiple hidden layers along with
%the input and output layer. But with abstract libraries, the user doesn't have
%any tools to inspect within the model.
%Furthermore, while connecting these APIs to build the neural network the 
%user has many places of single point failure starting from dimension mismatch, 
%wrong activation function usage as well creating hidden loops with 
%a performance overhead. 20 out of 385 questions for \keras are about training 
%time error 
%We have found 20 questions related to training time error out of 385 questions in \keras. 






==> interold.tex <==
We now describe the results of our inter-library analysis across all ten ML libraries
shown in \tabref{tbl:dataset}.
\figref{fig:interlib} shows the distribution of all the questions into different 
subcategories ordered from left to right following the leaves of the classification
tree shown in \figref{fig:classes}.
The observations are grouped based on the six stages of the ML pipeline shown in 
\figref{fig:steps}.

%In this section, we provide interlibrary analysis of the popular machine learning frameworks.  We see the distribution of all the questions into different subcategories ordered from left o right following the leaves of Figure \ref{fig:classes} is shown in Figure \ref{fig:interlib}. The observations are categorized as per the 6 stages of the pipeline that we are using for study.
%%\begin{itemize}
%%    \item All the library users face higher number of problems in model choice phase which includes creating the model by connecting different components and library features, choosing the right model for a particular problem
%%    \item Sklearn developers are happy because they have less problems on installation, platform, bugs etc. But other library users have often face a good volume of problems on installing, dependency related problems. This is because sklearn is developed as highly abstract library on top of \tensor or \theano backend and these issues are taken good care.
%%    \item Sklearn users face more problem at the prediction phase, evaluation phase, data preparation phase, and choice of hyper parameter phase because the library is highly abstract for a developer to go deeper and the glue code is also a source of major technical debt \cite{sculley2015hidden}. And this problem is faced more by the sklearn users to debug, maintain and find the reason of failure or sub optimal performance of the models.
%%    \item Tesnorflow users also have a lot of problems in using the library starting from installation of the use of a lot of APIs. \tensor users also face high volume of problems in model creation, choosing algorithm implemented in the library.
%%\end{itemize}
%%We now discuss different libraries depending on stages of machine learning pipeline.

\subsubsection{Data Preparation}
%\input{dataprep}
%For example we see in Figure \ref{fig:dataprep} a question asked by a \tensor developer about feeding some data to the library for doing transfer learning. Here the user is trying to use a pre-trained model to apply transfer learning into his own dataset. But he is facing problem due to the change of the input data. The user doesn't have the clue on how to feed a different type of data or tell the library that the input data is in different format.  
% When we take a closer look at the Figure \ref{fig:interlib} we observe the following things:
An analysis of \figref{fig:interlib}, and subsequent analyses of the dataset
reveals the following findings.

\paragraph*{\textbf{\weka, \mllib and \torch users face more difficulty in data preparation layer}} 
Their users have more difficulty to adapt to their data format and successfully feed data to the machine learning pipeline. We observe from \figref{fig:interlib} that these libraries have more than 20\% questions related to adapting data to the library. The major reason is that \weka and \mllib uses less popular data formats. \torch uses tensor but the APIs to load custom data, change types of tensors is not user friendly like \tensor and more vulnerable to error.

\paragraph*{\textbf{\keras, \scikit and \tensor users have more shape mismatch problems.}}
\keras, \scikit and \tensor all have close to 5\% of shape mismatch problems. In \keras and \tensor shape mismatch appears due to shape incompatibility of tensors at different layers. In \scikit shape mismatch appears due to shape or dimension mismatch of matrices or vectors. \scikit and \keras are abstract libraries where it is common for a developer to fail to track dimension requirement of different components given the input data. \tensor users also face shape mismatch related while passing tensors. In \tensor flow graph nodes are ops and edges are Tensors. Due to the lack of static feedback the users often mess with the strict requirement of dimensions. sometimes the dimension loss happens due to problematic computation done by some OP node.
%\paragraph*{\tensor, \caffe and \theano have less difficulty in data preparation stage}. 
%\tensor and \theano have in general less difficulty in data preparation stage compared to other libraries. These have close to 5\% difficulty in Adapting data which is still higher compared to all the subcategories we used to characterize the overall pipeline but less compared to adapting data phase of other libraries. 

\paragraph*{\textbf{Type mismatch problems}}.
Type mismatch problems range between 0-5\% in the libraries we studied. In \mahout, \torch and \ho type mismatch is almost negligible. But in other libraries type mismatch related problems appear more. These libraries need the data to be in a specific type, but the input data may not have the desired type.
These libraries in general doesn't provide any sanity check. 
%For example, often it happens an user read a CSV file and used that data for
%training. The data fields may be in String format while the library is asking
%for float, The labels may not be encoded from categorical variable using One hot
%encoding or some other encoding technique. And the libraries in general doesn't
%provide the verification or sanity check of these problems beforehand.

\paragraph*{\textbf{Data cleaning problems are more common in \scikit and \weka.}}
Problems that emanate from data cleaning phase are seen affecting more and causing more errors in \scikit and \weka. These libraries have close to 5\% questions that relate to data cleaning step. \tensor, \mllib are following \scikit and \weka having close to 2\% questions on data cleaning. Data cleaning problem appears more in these libraries because they provide abstracted APIs for data preparation that fail to catch missing and improper values.
% support and it sometimes mess up cleaning the values. Data cleaning problems like missing values, improper values are not caught beforehand and the error continues. 

% TODO: Revert this, if space available.
%\paragraph*{\textbf{Feature Selection and Feature extraction problems are more common in \scikit}}
%\scikit users have more questions on feature selection and feature extraction. One reason for this may be \scikit provides highly abstract functionalities for feature selection and the users don't have to observe the data themselves or do some preliminary exploratory analysis to find important features. But full transparency into the libraries execution and adequate introspection facilities are not available to help developers. \scikit library does provide APIs to select important features, extract features. These sometimes lead to improper feature selection or error due to misuse of API or improper preprocessing of data.  
%% When library is doing this it is sometimes creating confusion on using the APIs successfully, sometimes not giving the optimal results, sometimes throwing error. 
%%\begin{itemize}
%%    \item Data preparation is a major concern of the users of Apache Spark \mllib and \weka. When we see that the data format requirement of these libraries is totally different than most developers are acquainted with we can reason about it. \mllib demands data to be in RDD format which troubles a lot of developers to properly create the RDD format from input data in various format. Sometimes the conversion is corrupted making the whole process to be failed. \weka needs data in ARFF format which is also not a usual practice in other domains and less popular to the developers. So developers face difficulty in creating these formats from raw data. 
%%    \item Sklearn is highly abstract. That creates some additional technical debts. And we observe that data preparation stage creates some difficulty to the users of \scikit. Type related error, different encoding related problems often cause problem to these users. The program gives exception due to unwanted values, types etc. 
%%    \item \tensor and \caffe users have less difficulty in data preparation stage. But they have most problems related to the shape mismatch of multi dimensional vectors at different hidden layers due to improper data feeding or improper pre processing of data. 
%%    \item In general most library users have higher volume of problems in data preparation stage. Which can be reduced to a much higher degree with research and innovations from software engineering research. 
%%\end{itemize}

\subsubsection{Choosing model}
\input{chosemodel}
Recall that 
we classify the questions like choosing a right model for a problem domain that is implemented in the library, choosing from different overridden versions of a model creation function, strategy to create the model using library functionalities, etc, 
into this category. 
For example,
\figref{fig:chosemodel} shows a question where a developer is seeking help on the strategy to create a model using the library. Often the developer doesn't have sufficient understanding of the library to answer questions like ``how to connect or use library APIs to create KMeans algorithm."
An analysis of this category in \figref{fig:interlib} and additional investigation of dataset reveals the following findings.

\paragraph*{Deep learning libraries and libraries made for cluster have more model creation problems}
We see almost all the libraries have the higher number of questions in model creation category. Deep learning libraries like \keras, \caffe, and libraries for the cluster like Apache \mahout have more questions on model creation. Deep learning libraries consist of multiple layers and library code that builds the network but doesn't give hint to the users whether the API usage created a properly connected model, whether there is any connection gap between layers as well as what kind of network should be optimal given a problem is a concern. 
% Commenting the following paragraph to make space.
%\keras users have comparatively less questions than \caffe users. Because they remove the difficulty of designing the network schema like \caffe. The users can connect layers one after another to form the architecture by using the APIs. But still problems on successful connection of different layers create problem to some users.

%\paragraph*{\scikit users have more questions on model choice} In general,
%we see, all library users have the major percentage of difficulty in model
%creation stage. \scikit users have more questions related to selecting the
%best model compared to other libraries. This suggests a research path on
%suggesting the best model to users based on given dataset, features. Perhaps the
%library can help a developer select the best model.

\subsubsection{Training}
\label{subsec:training}
\input{training}

Next, we consider the training category. An example is presented in \figref{fig:training}
that illustrates a common trend for questions in this category: ML libraries generally do 
not provide enough diagnostics information. Other findings are the following.
%Figure \ref{fig:training} shows a question on training phase. The user is having difficulty in training a model and getting an exception but the user doesn't have the traceback on how to solve this exception and train the model successfully. 
%% Commenting out the above paragraph to make space.
%If we observe the chart in Figure \ref{fig:interlib} we notice and observe the following things:

\paragraph*{Training time error or exception happens more on \keras, \tensor, Sklearn, \mllib and \theano}
Around 5\% of questions for all of these libraries are about error thrown at training time.
Typically the developer has built the model following the documentation or theoretical knowledge but the training stops and unexpectedly throws errors or exceptions. The developer in most of the cases doesn't have sufficient diagnostics information to resolve those errors easily. 

% All these libraries have an error of around to 5\% at training time. When the user has built the model following the documentation or theoretical knowledge but the training stops throwing error/exception unexpectedly. The user in most of the cases doesn't have library feedbacks to resolve those errors easily. 

\paragraph*{Complex model creation but less training time error in \caffe}
Though the model creation is tightly coupled among different components in \caffe starting from designing the model schema in protobuf file to solver file with instructions to run the model, the training time errors are reduced. Interestingly compared to other libraries including deep learning libraries the number of questions about errors/exceptions is much less at training time. We believe that this could be because the developers have to take major care in designing the model which has a positive impact on using an error-free network for training.

\paragraph*{Choice of parameter related problems appear more in \torch and \caffe}
Compared to other libraries choice of parameter related problems are more in \torch and \caffe. Both these libraries have 
almost 10\% questions about this problem. \keras and \scikit are a close second, with around 5\% questions on parameter choice for training.

\paragraph*{In deep learning libraries like \torch, \caffe, \theano model conversion related questions are common}
In \torch 3/61, in \caffe 3/135, in \theano 5/191 questions specifically ask about reusing the model in a different environment. Model Conversion related questions are also seen in \weka, \scikit. 
We think that the primary reason for this is because training a deep learning model is often costly,
and thus developers are eager to reuse their training investments.
%Deep learning training is often costly. Through the concept of neural network or
%deep learning is not new, it lost interest in the 90s from the researchers due
%to computational cost needed for it. But due to the development of
%high-performance computing power deep learning has been growing very fast since
%last few years. This clearly indicates that people should be interested to reuse
%the model trained using one library to use in another library. This is why model
%conversion related questions are more seen in these deep learning libraries.
%Also, the model conversion is an important piece in transfer learning
%\cite{pan2010survey} which has been able to solve many interesting problems with
%great success \cite{kandaswamy2016high}. This suggests a deep software
%engineering research of the concepts of re-usability to be applied to machine
%learning model. Also, model conversion and reuse problem is present in \weka to a
%higher extent.


\subsubsection{Evaluation of the model}
%\input{evalaution}
%This phase includes choice and using of different evaluation strategy like cross-validation, performance of the trained model on the validation data, study model properties and present or visualize. 
%\paragraph*{\keras, \tensor, Sklearn, \weka have more problems in Evaluation stage}
%Model evaluation related problems appear more in \keras, \tensor, Sklearn and \weka. In \weka and Sklearn chosing the evalaution strategy or using the library provided evaluation utilities correctly is more common. In the deep learning libraries evaluating the layers of the model while learning, visualizing the learned model etc are more common along with evaluation strategies. 
Our findings for the Evaluation category are as follows.
% When we observe the Figure \ref{fig:interlib} we notice the following things at the evaluation stage. 
\paragraph*{\keras, \tensor, \scikit, \weka have more problems in Evaluation stage}
Model evaluation related problems appear more often in \keras, \tensor, \scikit, and \weka. In \weka and \scikit choosing the evaluation strategy or using the library provided evaluation utilities correctly is more common. In the deep learning libraries questions related to
evaluating the layers of the model while learning, visualizing the learned model, etc., are more common along with evaluation strategies. 
\subsubsection{Hyperparameter tuning}
%\input{hyperparam}
%In this section the initially chosen hyperparameters are updated or modified or some re choice of optional parameters are made. Figure \ref{fig:hyper} shows an example question in this stage.
Our findings for the hyperparameter tuning category are as follows.
\paragraph*{Sklearn users face more problems on hyperparameter tuning}
\scikit provides APIs that takes many optional parameters. The values of these optional parameters are set to a  default value and the users often face problem in tuning these parameters. Though the model works without these parameters, often to get the best accuracy wise choice and tuning of these parameters is necessary.
\subsubsection{Prediction}
%\input{prediction}
%In this section people see failure of the trained model performing poor on general or new coming data. Questions on making prediction from the trained model or loading pre-trained model are also added here. Figure \ref{fig:prediction} shows an example question in this phase.
Our findings for the prediction category are as follows.
\paragraph*{\weka, \keras and \scikit have more problems in the prediction stage}
\weka has the highest number of problems related to prediction. The library has built-in APIs along with a GUI based work flow system. Users just need to connect different components of the workflow. We observe that despite significant attempt to make machine learning and data mining user-friendly their users face a great deal of difficulty in prediction stage. \keras and \scikit also have a higher number of problems in the prediction stage. These libraries hide almost all of the details of machine learning from the user providing abstract APIs. Though abstract APIs ease the use of ML libraries, users of abstract APIs also get suboptimal performance in prediction stage. \weka and \keras have more than 10\% questions on prediction stage and \scikit has close to 7\% questions on prediction stage. 
%\subsection{Observations}
%Some important observations from the study are given below:
%\begin{enumerate}
%	\item Libraries that use an uncommon or new format of data creates more technical debt in data preparation layer. We can observe in Figure \ref{fig:interlib} that \weka and \mllib library users face more difficulty in the data preparation stage during adapting data to the machine learning pipeline. 
%	\input{ob1}
%	As we observe in a sample question in Figure \ref{fig:ob1weka} that the user is trying to use a dataset from a well known machine learning dataset repository provided by UCI (University of California at Irvine). Usually these datasets are pre processed to do machine learning and importing these datasets can be done directly. But an user of \weka user is not able to successfully adapt the dataset to the library for training due to the failure of conversion to ARFF format needed by the library. Similarly the library Apache spark \mllib users also have a higher percentage of difficulties faced by the users at the data preparation stage. As it uses RDD format of data which is less popular to the users. Adapting the data for the library, converting from popular data formats the the format required or preferred by the library are some common problems faced by the users when the library uses less popular data formats.
%	\item  Sklearn library provides a good set of functionalities to do feature selection and feature extraction. 
%	\input{ob2}
%	For example in Figure \ref{fig:ob2sklearn} the user is facing some problem in using the built in API to select features from the data for building a model. 
%	Users also face difficulties in encoding data, cleaning data, shuffling and splitting of data, extracting features from data, data cleaning etc. The users face mainly problems related to exceptions, non satisfactory results.
%	\item Libraries that use higher abstraction create additional difficulty for users in model creation. 
%	\input{ob3}
%	For example in Figure \ref{fig:ob3} an user is trying to use the APIs provided by the library to build a model but is getting error in building the model correctly. 
%	The abstract libraries hide all the crafting techniques in building machine learning models from the users. That makes making the model interesting and easy to use to average users but can be reasons of failure to make the model working or making the best model. This problem is more common among the users of \scikit and \keras. 
%	\item Lack of rich and interactive debugging options cause a lot of difficulties 
%	in building machine learning models. When some model is throwing exception at training time, some model is not converging or learning as the iteration of training goes on, some model is not predicting well, some model creation is not correct and producing garbage results, some model is not performing well for a particular instance of a problem and a lot other problems faced by developers can ne minimized to a great extent with effective debugging options. \tensor team has attempted to add debugging options through TensorDebug \cite{tdebug}. The concept of debugging some tasks by implementing machine learning with the help of probabilistic programming is presented by the authors in \cite{chakarov2016debugging}.
%	\item \tensor has comparatively less difficulties in data preparations stage. There are some difficulties in adapting TFRecords or storing data in this format. But still \tensor provides multiple options to read and store data. And the dataset for using in the machine learning pipeline is stored as dataset of elements of same size and each element can contain on or more Tensor objects. Each Tensor object also has Type information and shape information added with it. 
%	Using Tensor object and providing functionalities to read raw data and forming dataset using Tensor objects reduce errors, adapting or data cleaning related problems. An example of how the dataset is represented as tensor from a random uniform matrix of 4*10 size is given in the following code snippet:
%	\input{tensor}
%	We see that the dataset is read and parsed as tensor by the library with type and shape information. It provides easier adapting of data as well as debugging any dataset related problem by tensor debug. \torch and \theano also uses tensors as their data structure. Although they have comparatively less problems in data preparation stage but the data adapting and loading APIs create slight difficulties compared to \tensor in these libraries. 
%	\item \tensor popularity is growing very fast since the inception of the library in November 2015. It provides some model evaluation and monitoring of the model at run time through visual interface using tensorboard, it provides some debugging functionality using tensordebug, it uses Tensor data structure to represent its data internally and flow data to different components in the pipeline. Its developers have some questions on handling sparse tensor data. And the monitoring of sparseness of the tensor at different stage is not yet supported. Analysis of sparsity of tensors at different stages of the pipeline and then optimizing the computation can be future work. And also the storing technique of different types of sparse tensors can be a great addition. Some research on the line has been proposed and presented by the authors in \cite{kjolstad2017tensor}.
%	
%	\item Converting model trained using one library and using it another library is a common problem. For example lets consider someone has trained an SVM model on a particular dataset D. The user then wants to load the model in \weka and use that for future prediction. Some libraries provide some support to convert model for using with other library but those are not always good. But some libraries dont have that support and the trained model can not be reused with other platforms.
%	\item All the library users face comparatively higher difficulty in model creation stage. Deep learning library users have comparatively more difficulty in the model creation stage. Almost 30\% of the questions asked by deep learning library users on stackoverflow where score is at least 5 is on choice of model stage. Model of choice contains topics related to model creation, selecting best model, converting model etc.
%	\item Hyperparameter tuning related questions are comparatively more to the \scikit users. Usually \scikit api designs take a lot of optional parameter. For example we see an API to create AdaBoostClassifier below with a lot of optional parameters initialized by default to None.
%	\input{sklearn}
%	And finding good value of these parameters and tuning these parameters to make the 
%	best model, avoid over-fitting are seen more among \scikit developers. 
%	There has been some github issues filed to the repository of \scikit and the reason was the user was not able to trace why the model is not showing expected accuracy. And the answer was tuning hyper parameters. For example against an issue submitted to the official repository the quick and small answer from an expert was like the following Figure \ref{fig:tune}.
%	\input{tune}
%	\item \keras a highly abstract deep learning library users get comparatively higher error at runtime. 
%	\input{keraserr}
%	For example in Figure \ref{fig:ob6} the user has built the model succesfully yet the user gets error at run time. The major reason is that building deep learning model needs to successfully connect multiple hidden layers along with the input and output layer. But using abstract libraries the user doesn't have any static analysis tool to check where the mistake has happened.
%		
%	\item \keras and Sklearn are highly abstract and hide all the details of machine learning implementations from the users. This sometimes creates some untraceable suboptimal performance in prediction. Because the user doesn't have the way to trace where the model was not functioning correctly, whether some over-fitting problem happened. For example an user has built a model successfully and got training successful with satisfactory training accuracy. But when the new data is given input to the model for prediction the prediction accuracy is very low. In most of these cases the user even doesn't have any way to trace the reason of these sub-optimal performance. So abstracting the functionalities and making more general users to practice machine learning doesn't ensure that they are doing machine learning with satisfactory success.
%	\item The libraries that are specialized for doing machine learning in the cluster have more difficulty in the choice of model phase specially in model creation. For example \mllib, \mahout are libraries to do large scale machine learning in cluster.
%	\input{mahout}
%	 The users of these libraries face higher difficulties in model creation, running model in parallel following map-reduce paradigm, selecting the appropriate model. For example in Figure \ref{fig:mahout} the user is trying to build a model to build his custom model but he has no idea on how can he create that model. The top voted answer suggested how can the person achieve his goal  by combining a multiple ideas as well as how the performance can be optimized using cluster. 
%	 \item \caffe users have problems in model creation due to the dependency of model on multiple files. To create a model successfully one needs to make a schema file in protobuf format, create a solver file and write codes in c++ or python to build the model. For example this tutorial https://medium.com/machine-learning-world/using-caffe-with-your-own-dataset-b0ade5d71233 states multiple steps needed to build a model successfully using \caffe and python. This gives us some intuition that the framework where the model depends on multiple things or there are more than one way of creating the same model creates some technical debt in the model creation phase.
%	 \item The machine learning frameworks have APIs that are very often misused. The general guideline of API design is such that it is difficult to misuse the API. But we have seen a lot of the problems faced by machine learning developers are due to using the API in an improper way. This problem happens in the APIs at almost all stages of the pipeline starting from data preparation to prediction. 
%	 \input{apimis}
%	 For example we see in Figure \ref{fig:apimis}a a question asked by a user that, his training takes much time or longer number of iterations to get a certain training accuracy. In one fit API he is able to achieve the accuracy only in 5 iterations where in other API the  user needs 60 iterations to reach the same accuracy. Everything is working fine, without any error and eventually reaching the same accuracy also. But still the user is astound by almost 12 times higher number of iterations in using the second API. And the ans in Figure \ref{fig:apimis}b suggest that the second API needs the data to shuffled properly before passing to the API in every iteration. And changing only that part solved the performance problem.
%	 
%	 This kind of API misuse is very common in machine learning API at all stages. It causes problems on failure to find important features, properly preparing the dataset, performance, over-fitting, suboptimal prediction performance, error, warnings etc. 
%	 \item Shape mismatch of tensors at different layers is also a common problem among the libraries that use tensors or matrices. This problem is seen more commonly in deep learning library. For example when tensors pass from layer $i$ to layer $j$ in the network then there should be some size compatibility otherwise it can raise exception during training and even it can fail at the very starting of the runtime. 
%	 \input{shape}
%	 For example we see in Figure \ref{fig:shape} a sample question on shape mismatch. 
%	 \item Type mismatch is also a common problem faced by developers. The training stops due to this type mismatch problem. 
%	 \input{type}
%	 For example Figure \ref{fig:type} shows a question on type mismatch. 
%\end{enumerate}




==> intracharts.tex <==
\begin{figure*}[t]
	\centering
	\begin{subfigure}[t]{0.31\textwidth}
		 \centering
		\includegraphics[height=1in,width=\linewidth]{tensorflow}
		\vspace{-1em}
		\caption{\tensor}
	\end{subfigure} %\hfill
	\begin{subfigure}[t]{0.31\textwidth}
		\centering
		\includegraphics[height=1in,width=\linewidth]{sklearn}
		\vspace{-1em}
		\caption{\scikit}
	\end{subfigure} %\hfill
	\begin{subfigure}[t]{0.31\textwidth}
		\centering
		\includegraphics[height=1in,width=\linewidth]{keras}
		\vspace{-1em}
		\caption{\keras}
	\end{subfigure} % \hfill
	\begin{subfigure}[t]{0.31\textwidth}
		\centering
		\includegraphics[height=1in,width=\linewidth]{weka}
		\vspace{-1em}
		\caption{\weka}
	\end{subfigure} % \hfill
	\begin{subfigure}[t]{0.31\textwidth}
		\centering
		\includegraphics[height=1in,width=\linewidth]{caffe}
		\vspace{-1em}
		\caption{\caffe}
	\end{subfigure} % \hfill
	\begin{subfigure}[t]{0.31\textwidth}
		\centering
		\includegraphics[height=1in,width=\linewidth]{theano}
		\vspace{-1em}
		\caption{\theano}
	\end{subfigure} %\hfill
	\begin{subfigure}[t]{0.31\textwidth}
		\centering
		\includegraphics[height=1in,width=\linewidth]{mllib}
		\vspace{-1em}
		\caption{\mllib}
	\end{subfigure} % \hfill
	\begin{subfigure}[t]{0.31\textwidth}
		\centering
		\includegraphics[height=1in,width=\linewidth]{torch}
		\vspace{-1em}
		\caption{\torch}
\end{subfigure} % \hfill
	\begin{subfigure}[t]{0.31\textwidth}
		\centering
		\includegraphics[height=1in,width=\linewidth]{apachemahout}
		\vspace{-1em}
		\caption{\mahout}
	\end{subfigure} % \hfill
	\begin{subfigure}[t]{0.31\textwidth}
		\centering
		\includegraphics[height=1in,width=\linewidth]{h2o}
		\vspace{-1em}
		\caption{\ho}
	\end{subfigure} % \hfill
	\vspace{-1em}
	\caption{Intra library distribution of \sof questions into different subcategories. The subcategories are labeled in the x axis sequentially from Figure 2 leaf nodes.}
	\label{fig:intra}
\end{figure*}



==> intranew.tex <==


\subsubsection{\caffe} 

As shown in \tabref{tbl:cat}, most of the questions about \caffe involve 
\textbf{modeling (32\%)} and \textbf{training (24\%)}.
%\caffe shows the maximum percentage of questions on 
%choice of model and training stages both with 27\% and having the most 
%significant part of the questions on those two stages. 
The third largest category is data preparation (14\% of the total questions).
% The data preparation stage is the next to these two stages having 14\% of the 
% total questions. 
The largest subcategory of questions for \caffe is
\textbf{model creation} with \textbf{26.52\%} questions.
% Among the subcategories, we can see, from 
% \tabref{tbl:subcat}, that \caffe has the most share of questions on \textbf{model creation} with \textbf{26.52\%}. 
%Questions related to data adapting appear 9.85\% of the time and prediction accuracy related questions appear 5\%. 
Even though prediction stage has only 6\% of the questions at the top-level 
category, one of its subcategory, prediction accuracy, is in the top-5 most 
concerned problems. 
%From the statistical analysis of outliers we see that 
%\caffe is outlier in the subcategory \textbf{bug}. This could imply that \textbf{automatic 
%bug detection technique for this library may be of great help to its users}. 

\subsubsection{\ho}

\ho is the library that has the least amount of data from \sof among the 10 
chosen libraries for analysis with only 20 questions. 
%Therefore, making very strong claims on this sparse data can be risky. 
%From the distribution of questions about this library we see almost 
41\% of them are about data preparation that suggests that 
the design of data preparation stage can be improved for this library
or tools could be made to ease data preparation. In the 
subcategories, we see data adaptation related question appear 35.29\% of the 
time and the next major subcategory is model creation with 17.64\%. From the 
outlier analysis, \ho has much more questions in the output interpretation 
and tuning strategy selection than other libraries. That would mean that its 
library users could benefit from \textbf{improved APIs for hyper-tuning 
strategy and displaying well-formatted results}.

\subsubsection{\keras}

\keras is a popular deep learning library which uses \tensor or \theano as 
backend. \keras provides a collection of abstract APIs that hide the details of 
\tensor or \theano computation. This library has most of the questions on 
modeling (28\%), followed by training (25\%) and data preparation (16\%). In 
the subcategories, the majority of posts are on model creation (25.88\%), 
and several others with similar contributions: data adaptation (7.90\%), 
prediction accuracy (6.81\%), performance (6.27\%), shape mismatch (5.50\%), 
error/exception (5.50\%) and parameter selection (5.50\%). 

The result implies that the abstraction in \keras does not help reduce the 
difficulty with modeling in \keras. More research is needed on the 
\textbf{abstraction strategy for ML libraries}. %
%We also see data preparation related problems also appear in high volume 
%instead of providing the APIs for data preparation and adaptation raw data to 
%the pipeline. Performance becomes an issue related to memory/time as the user 
%has less information what is going at the backend. Error/Exception at 
%training time seems to show more with the abstraction. 
%
%For the outlier analysis, \keras seems to have more problems with shape 
%mismatch, output interpretation and model reuse than other libraries. Even 
%though abstraction reduces the amount of written code, constructing deep 
%neural networks layer by layer using the abstraction is not quite intuitive 
%yet. These gives indication of an unique abstraction model in engineering 
%these libraries. 

\subsubsection{\mahout}
\findings{\mahout has abnormally high percentage of questions about model 
	creation which is outlier compared to other libraries}{
	Model creation in parallel machine learning libraries is difficult. 
	%Abstract model selection APIs in \scikit didn't reduce the 
	%difficulties in model creation and model selection. Which gives intuition 
	%about an ML oriented abstraction for designing model creation and model 
	%selection APIs.
}
Model creation in parallel machine learning libraries is difficult which is revealed in Finding 15. 
Apache \mahout is a specialized library for performing ML 
on clusters. This library has the most questions in modeling 
stage with 44\%, most of which are in model creation, followed by 
data preparation with 17\%. This indicates that creation of model on 
clusters is comparatively more difficult. Other than model creation the 
prominent subcategories for this library are data adaptation (14.58\%), 
prediction accuracy (4.2\%) and error/exception(4.2\%). 
%From the outlier analysis we see that \mahout is an outlier in the model 
%creation sub category indicating research directions in parallel machine learning. 
The result suggests that \textbf{much work is still needed in distributed ML}. 

\subsubsection{\mllib}

\mllib is another prominent library for distributed ML. This 
library has the highest percentage of questions on data preparation (33\%). %
A reason could be that \mllib uses a special data structure called 
resilient distributed datasets (RDD). Most of the time developers need to be 
comfortable with this format of data while using this library. \textbf{Using 
a new data format may also create new technical difficulty in data 
preparation stage}. The other prominent category is modeling (29\%). 
Among the subcategories, the prominent subcategories are data adaptation 
(25.20\%), model creation (23.52\%) and error/exception (5.88\%). 
% COMMENT-HR: What is the implication of the last sentence? This ends abruptly.
%
%These statistics show \mllib has major weakness in the data preparation stage 
%and also model creation. As we already discussed earlier parallel machine 
%learning libraries tend to show more problems in the model creation part. 
%\mllib shows additional and the largest share of difficulties in the data 
%preparation stage due to the use of less popular data format. 


\subsubsection{\scikit}

\scikit is a popular ML library in Python. Though it is not 
used for deep learning, its use for regression, supervised and unsupervised 
learning, and recommendation related tasks are well known. This library 
provides abstract APIs that hides the details of ML.
In our study, the majority of questions about \scikit were about data 
preparation (26\%), modeling (25\%), and training (18\%).
%it has 26\% of questions in the data preparation, 
%25\% in the modeling and 18\% in the training stage taking the major share of 
%questions. 
Here again, we could see that abstractions does not resolve the 
problems on modeling, data preparation and training for this library either. 
% COMMENT-HR: Why do we believe the last sentence? 
%When we go deeper into subcategories, we see that the prominent subcategories 
%are model creation (21.37\%), featuring (9.34\%), data adaptation (8.64\%) and 
%prediction accuracy (5.25\%). 
%%We see that feature selection is a major problem after model creation. 
%Though \scikit provides a good number of abstract APIs for feature selection 
%its usage is still problematic. High number of questions on prediction accuracy 
It would suggest that \textbf{hiding all the details of ML 
tasks using abstract APIs might create difficulties in tracing and debugging} 
when the models are not learning properly or over-fitting. 

\findings{\scikit has the highest number of posts on feature selection/extraction 
	subcategory (9.34\%).}{Blackbox abstraction for feature selection/extraction 
	APIs may not be suitable for ML libraries.} 
Finding 16 suggest that, blackbox abstraction for feature selection/extraction 
APIs may not be suitable for ML libraries.
We also notice from outlier analysis that \scikit has more questions in model 
creation and tuning parameter selection than others. \scikit provides a lot 
of optional parameters to be selected in their APIs, whose values are hard to 
select yet affect accuracy. That could be the reason why its users have more 
difficulties in selecting parameters. This calls for \textbf{research 
on designing APIs for parametric ML}. 

\findings{\scikit has abnormally high percentage of questions about model 
	creation compared to other libraries due to its lack of guidelines for model 
	selection.}{Recommendation support would be helpful in selecting models.
	%Abstract model selection APIs in \scikit didn't reduce the 
	%difficulties in model creation and model selection. Which gives intuition 
	%about an ML oriented abstraction for designing model creation and model 
	%selection APIs.
}
We see from Finding 17, recommendation support would be helpful in selecting models.
Surprisingly though parameter selection and hyper parameter tuning is one of the fundamentals problems in ML, there is less discussion about it among the programmers. But \scikit is an outlier in this category indicating the way \scikit APIs provide abstraction for hyper parameter selection creates difficulty among the programmers. 

%\findings{\scikit has more difficulty in hyper parameter tuning compared to 
%	other libraries}{Due to the presence of a lot of optional parameters in the 
%	APIs, the tuning of these parameters is more problematic than other libraries. 
%	This gives intuition of having tools to suggest parameters that may have 
%	effect on a particular model and particular problem. }
\subsubsection{\tensor}

This library, which is actively maintained by Google, covers the highest 
percentage of questions in \sof. This library comparatively faces less 
difficulty in data preparation (16\%) but the issues in modeling and training 
take the higher share (27\% and 21\%, respectively). 
%Modeling stage is next with 20\%. 
If we go deeper into subcategories, we see that model creation (23\%), data 
adaptation (9.22\%), error/exception (5.32\%), evaluation strategy (5.24\%), 
performance (4.87\%) and prediction accuracy (3.97\% ) are the dominant subcategories. 
Our conjecture is that \textbf{automatic static analysis and verification 
would be helpful in designing tensor networks}.
% COMMENT-HR: Why do we believe the last sentence? 
%This gives us intuition that model creation in \tensor needs some static 
%analysis support to help the developers. Also there should be some tools to 
%automatically verify the design of the network. 


\subsubsection{\theano}

\theano is a deep learning library that shows major difficulties in modeling 
stage (27\%). Data preparation (17\%) and training (16\%) follow next. 
Among the subcategories, model creation (23.43\%), data adaptation (10.41\%) 
and error/exception (5.72\%) are the most problematic subcategories. This 
suggests that, besides tool support for data processing and data adaptation, 
\textbf{runtime checkers/verifiers for \theano models} are also needed. 

\subsubsection{\torch}

\torch is also a specialized deep learning library. For this library, 
modeling (33\%), data preparation (23\%) and training (20\%) show 
the highest levels of difficulties. 
Among the subcategories, 
data adaptation (22.95\%) and model creation (22.95\%) are the most problematic subcategories. 
%This indicates this library can be improved a lot by paying attention to the data 
%preparation APIs. Model creation (22.95\%) has almost the same volume of 
%posts as in the data adaptation subcategory. 
%Choice of parameter (8.2\%) is 
%dominant for this library which indicates research on designing APIs for 
%parametric deep learning can be of great help. 

\subsubsection{\weka}

\weka is a popular data mining and ML library for Java. 
This library has the highest volume of posts about the data 
preparation (30\%), most of which are about data adaptation. This is much 
higher than the median for data preparation of all the libraries (20\%). 
\weka uses a custom data format called ARFF.
This would suggest that using a custom data format introduces 
additional technical difficulty in the data preparation stage like in \mllib. So 
\textbf{when a custom data format is used automatic conversion with 
correctness guarantee should also be provided} to the developers. This 
can be a direction of research for both software and 
data engineering researchers. 
%
The next dominant stage is modeling (20\%). Training stage for \weka 
looks comparatively better: 12\% compared to the median among all libraries of 18\%. 

%If we go deeper into subcategories, 
%we see that, other than data adaptation and model creation, the next prominent 
%subcategories are evaluation strategy (8.54\%) and prediction accuracy (8.54\%). 
%This indicates that instead of providing good number of abstract APIs the 
%evaluation strategy still causes difficulty. And the prediction accuracy is 
%also a problem due to the high degree of abstraction the the traditional way. 
%Again indicating research on new abstraction model for engineering machine 
%learning libraries. 

The discussion and findings in this section along with the key findings shown in box shows there are libraries like \mahout, \scikit, \caffe, \torch that face problem in model creation. \scikit has problems in model and parameter selection. \weka and \mllib have more difficulty in the data preparation stage. 
%Evaluation, Tuning and Prediction stage seems to be equally difficult among all the libraries. And Model creation, Data preparation, Training form another group with hig

==> intraold.tex <==
We first study the strengths and weaknesses of different ML libraries 
in terms of each of the top-level categories defined in \figref{fig:classes}.

% We study different libraries and see the strong and weak part of 
% different libraries at different stages of machine learning in terms 
% of developers difficulty. 

%\input{Intra}

\input{intranew}
\input{interlibanalysis}
\subsubsection{Grouping libraries} 
We studied the libraries to see if there is some similarity of patterns among the libraries compared by the distribution of problems at different stages. 
\input{correlationoflibs}
From the above chart we group the libraries into the following categories
\textbf{Group 1}  \weka, \ho, \scikit, \mllib form a strong correlated group with correlation coefficient greater than 0.84 between the pairs. Other than \ho other libraries in this category are not used for deep learning. This gives us implication that the problems appearing in these libraries have some correlation and the difficulties one one library can be described by the difficulty of other libraries in the group.

\textbf{Group 2} \torch, \keras, \theano and \tensor form another group with strong correlation of more than 0.86 between the pairs. These libraries are specialized for deep learning. This gives us implication that deep study of one library can also be useful in the analysis for other deep learning libraries. That means that the problems are cross related to the libraries,
%\input{internew}

\subsection{Inter Library Analysis}

We now describe the results of our inter-library analysis across all ten ML libraries
shown in \tabref{tbl:dataset}.
\figref{fig:interlib} shows the distribution of all the questions into different 
subcategories ordered from left to right following the leaves of the classification
tree shown in \figref{fig:classes}.
The observations are grouped based on the six stages of the ML pipeline shown in 
\figref{fig:steps}.

%In this section, we provide interlibrary analysis of the popular machine learning frameworks.  We see the distribution of all the questions into different subcategories ordered from left o right following the leaves of Figure \ref{fig:classes} is shown in Figure \ref{fig:interlib}. The observations are categorized as per the 6 stages of the pipeline that we are using for study.
%%\begin{itemize}
%%    \item All the library users face higher number of problems in model choice phase which includes creating the model by connecting different components and library features, choosing the right model for a particular problem
%%    \item Sklearn developers are happy because they have less problems on installation, platform, bugs etc. But other library users have often face a good volume of problems on installing, dependency related problems. This is because sklearn is developed as highly abstract library on top of \tensor or \theano backend and these issues are taken good care.
%%    \item Sklearn users face more problem at the prediction phase, evaluation phase, data preparation phase, and choice of hyper parameter phase because the library is highly abstract for a developer to go deeper and the glue code is also a source of major technical debt \cite{sculley2015hidden}. And this problem is faced more by the sklearn users to debug, maintain and find the reason of failure or sub optimal performance of the models.
%%    \item Tesnorflow users also have a lot of problems in using the library starting from installation of the use of a lot of APIs. \tensor users also face high volume of problems in model creation, choosing algorithm implemented in the library.
%%\end{itemize}
%%We now discuss different libraries depending on stages of machine learning pipeline.

\subsubsection{Data Preparation}
%\input{dataprep}
%For example we see in Figure \ref{fig:dataprep} a question asked by a \tensor developer about feeding some data to the library for doing transfer learning. Here the user is trying to use a pre-trained model to apply transfer learning into his own dataset. But he is facing problem due to the change of the input data. The user doesn't have the clue on how to feed a different type of data or tell the library that the input data is in different format.  
% When we take a closer look at the Figure \ref{fig:interlib} we observe the following things:
An analysis of \figref{fig:interlib}, and subsequent analyses of the dataset
reveals the following findings.

\paragraph*{\textbf{\weka, \mllib and \torch users face more difficulty in data preparation layer}} 
Their users have more difficulty to adapt to their data format and successfully feed data to the machine learning pipeline. We observe from \figref{fig:interlib} that these libraries have more than 20\% questions related to adapting data to the library. The major reason is that \weka and \mllib uses less popular data formats. \torch uses tensor but the APIs to load custom data, change types of tensors is not user friendly like \tensor and more vulnerable to error.

\paragraph*{\textbf{\keras, \scikit and \tensor users have more shape mismatch problems.}}
\keras, \scikit and \tensor all have close to 5\% of shape mismatch problems. In \keras and \tensor shape mismatch appears due to shape incompatibility of tensors at different layers. In \scikit shape mismatch appears due to shape or dimension mismatch of matrices or vectors. \scikit and \keras are abstract libraries where it is common for a developer to fail to track dimension requirement of different components given the input data. \tensor users also face shape mismatch related while passing tensors. In \tensor flow graph nodes are ops and edges are Tensors. Due to the lack of static feedback the users often mess with the strict requirement of dimensions. sometimes the dimension loss happens due to problematic computation done by some OP node.
%\paragraph*{\tensor, \caffe and \theano have less difficulty in data preparation stage}. 
%\tensor and \theano have in general less difficulty in data preparation stage compared to other libraries. These have close to 5\% difficulty in Adapting data which is still higher compared to all the subcategories we used to characterize the overall pipeline but less compared to adapting data phase of other libraries. 

\paragraph*{\textbf{Type mismatch problems}}.
Type mismatch problems range between 0-5\% in the libraries we studied. In \mahout, \torch and \ho type mismatch is almost negligible. But in other libraries type mismatch related problems appear more. These libraries need the data to be in a specific type, but the input data may not have the desired type.
These libraries in general doesn't provide any sanity check. 
%For example, often it happens an user read a CSV file and used that data for
%training. The data fields may be in String format while the library is asking
%for float, The labels may not be encoded from categorical variable using One hot
%encoding or some other encoding technique. And the libraries in general doesn't
%provide the verification or sanity check of these problems beforehand.

\paragraph*{\textbf{Data cleaning problems are more common in \scikit and \weka.}}
Problems that emanate from data cleaning phase are seen affecting more and causing more errors in \scikit and \weka. These libraries have close to 5\% questions that relate to data cleaning step. \tensor, \mllib are following \scikit and \weka having close to 2\% questions on data cleaning. Data cleaning problem appears more in these libraries because they provide abstracted APIs for data preparation that fail to catch missing and improper values.
% support and it sometimes mess up cleaning the values. Data cleaning problems like missing values, improper values are not caught beforehand and the error continues. 

% TODO: Revert this, if space available.
%\paragraph*{\textbf{Feature Selection and Feature extraction problems are more common in \scikit}}
%\scikit users have more questions on feature selection and feature extraction. One reason for this may be \scikit provides highly abstract functionalities for feature selection and the users don't have to observe the data themselves or do some preliminary exploratory analysis to find important features. But full transparency into the libraries execution and adequate introspection facilities are not available to help developers. \scikit library does provide APIs to select important features, extract features. These sometimes lead to improper feature selection or error due to misuse of API or improper preprocessing of data.  
%% When library is doing this it is sometimes creating confusion on using the APIs successfully, sometimes not giving the optimal results, sometimes throwing error. 
%%\begin{itemize}
%%    \item Data preparation is a major concern of the users of Apache Spark \mllib and \weka. When we see that the data format requirement of these libraries is totally different than most developers are acquainted with we can reason about it. \mllib demands data to be in RDD format which troubles a lot of developers to properly create the RDD format from input data in various format. Sometimes the conversion is corrupted making the whole process to be failed. \weka needs data in ARFF format which is also not a usual practice in other domains and less popular to the developers. So developers face difficulty in creating these formats from raw data. 
%%    \item Sklearn is highly abstract. That creates some additional technical debts. And we observe that data preparation stage creates some difficulty to the users of \scikit. Type related error, different encoding related problems often cause problem to these users. The program gives exception due to unwanted values, types etc. 
%%    \item \tensor and \caffe users have less difficulty in data preparation stage. But they have most problems related to the shape mismatch of multi dimensional vectors at different hidden layers due to improper data feeding or improper pre processing of data. 
%%    \item In general most library users have higher volume of problems in data preparation stage. Which can be reduced to a much higher degree with research and innovations from software engineering research. 
%%\end{itemize}

\subsubsection{Choosing model}
\input{chosemodel}
Recall that 
we classify the questions like choosing a right model for a problem domain that is implemented in the library, choosing from different overridden versions of a model creation function, strategy to create the model using library functionalities, etc, 
into this category. 
For example,
\figref{fig:chosemodel} shows a question where a developer is seeking help on the strategy to create a model using the library. Often the developer doesn't have sufficient understanding of the library to answer questions like ``how to connect or use library APIs to create KMeans algorithm."
An analysis of this category in \figref{fig:interlib} and additional investigation of dataset reveals the following findings.

\paragraph*{Deep learning libraries and libraries made for cluster have more model creation problems}
We see almost all the libraries have the higher number of questions in model creation category. Deep learning libraries like \keras, \caffe, and libraries for the cluster like Apache \mahout have more questions on model creation. Deep learning libraries consist of multiple layers and library code that builds the network but doesn't give hint to the users whether the API usage created a properly connected model, whether there is any connection gap between layers as well as what kind of network should be optimal given a problem is a concern. 
% Commenting the following paragraph to make space.
%\keras users have comparatively less questions than \caffe users. Because they remove the difficulty of designing the network schema like \caffe. The users can connect layers one after another to form the architecture by using the APIs. But still problems on successful connection of different layers create problem to some users.

%\paragraph*{\scikit users have more questions on model choice} In general,
%we see, all library users have the major percentage of difficulty in model
%creation stage. \scikit users have more questions related to selecting the
%best model compared to other libraries. This suggests a research path on
%suggesting the best model to users based on given dataset, features. Perhaps the
%library can help a developer select the best model.

\subsubsection{Training}
\label{subsec:training}
\input{training}

Next, we consider the training category. An example is presented in \figref{fig:training}
that illustrates a common trend for questions in this category: ML libraries generally do 
not provide enough diagnostics information. Other findings are the following.
%Figure \ref{fig:training} shows a question on training phase. The user is having difficulty in training a model and getting an exception but the user doesn't have the traceback on how to solve this exception and train the model successfully. 
%% Commenting out the above paragraph to make space.
%If we observe the chart in Figure \ref{fig:interlib} we notice and observe the following things:

\paragraph*{Training time error or exception happens more on \keras, \tensor, Sklearn, \mllib and \theano}
Around 5\% of questions for all of these libraries are about error thrown at training time.
Typically the developer has built the model following the documentation or theoretical knowledge but the training stops and unexpectedly throws errors or exceptions. The developer in most of the cases doesn't have sufficient diagnostics information to resolve those errors easily. 

% All these libraries have an error of around to 5\% at training time. When the user has built the model following the documentation or theoretical knowledge but the training stops throwing error/exception unexpectedly. The user in most of the cases doesn't have library feedbacks to resolve those errors easily. 

\paragraph*{Complex model creation but less training time error in \caffe}
Though the model creation is tightly coupled among different components in \caffe starting from designing the model schema in protobuf file to solver file with instructions to run the model, the training time errors are reduced. Interestingly compared to other libraries including deep learning libraries the number of questions about errors/exceptions is much less at training time. We believe that this could be because the developers have to take major care in designing the model which has a positive impact on using an error-free network for training.

\paragraph*{Choice of parameter related problems appear more in \torch and \caffe}
Compared to other libraries choice of parameter related problems are more in \torch and \caffe. Both these libraries have 
almost 10\% questions about this problem. \keras and \scikit are a close second, with around 5\% questions on parameter choice for training.

\paragraph*{In deep learning libraries like \torch, \caffe, \theano model conversion related questions are common}
In \torch 3/61, in \caffe 3/135, in \theano 5/191 questions specifically ask about reusing the model in a different environment. Model Conversion related questions are also seen in \weka, \scikit. 
We think that the primary reason for this is because training a deep learning model is often costly,
and thus developers are eager to reuse their training investments.
%Deep learning training is often costly. Through the concept of neural network or
%deep learning is not new, it lost interest in the 90s from the researchers due
%to computational cost needed for it. But due to the development of
%high-performance computing power deep learning has been growing very fast since
%last few years. This clearly indicates that people should be interested to reuse
%the model trained using one library to use in another library. This is why model
%conversion related questions are more seen in these deep learning libraries.
%Also, the model conversion is an important piece in transfer learning
%\cite{pan2010survey} which has been able to solve many interesting problems with
%great success \cite{kandaswamy2016high}. This suggests a deep software
%engineering research of the concepts of re-usability to be applied to machine
%learning model. Also, model conversion and reuse problem is present in \weka to a
%higher extent.


\subsubsection{Evaluation of the model}
%\input{evalaution}
%This phase includes choice and using of different evaluation strategy like cross-validation, performance of the trained model on the validation data, study model properties and present or visualize. 
%\paragraph*{\keras, \tensor, Sklearn, \weka have more problems in Evaluation stage}
%Model evalaution related problems appear more in \keras, \tensor, Sklearn and \weka. In \weka and Sklearn chosing the evalaution strategy or using the library provided evaluation utilities correctly is more common. In the deep learning libraries evaluating the layers of the model while learning, visualizing the learned model etc are more common along with evaluation strategies. 
Our findings for the Evaluation category are as follows.
% When we observe the Figure \ref{fig:interlib} we notice the following things at the evaluation stage. 
\paragraph*{\keras, \tensor, \scikit, \weka have more problems in Evaluation stage}
Model evaluation related problems appear more often in \keras, \tensor, \scikit, and \weka. In \weka and \scikit choosing the evaluation strategy or using the library provided evaluation utilities correctly is more common. In the deep learning libraries questions related to
evaluating the layers of the model while learning, visualizing the learned model, etc., are more common along with evaluation strategies. 
\subsubsection{Hyperparameter tuning}
%\input{hyperparam}
%In this section the initially chosen hyperparameters are updated or modified or some re choice of optional parameters are made. Figure \ref{fig:hyper} shows an example question in this stage.
Our findings for the hyperparameter tuning category are as follows.
\paragraph*{Sklearn users face more problems on hyperparameter tuning}
\scikit provides APIs that takes many optional parameters. The values of these optional parameters are set to a  default value and the users often face problem in tuning these parameters. Though the model works without these parameters, often to get the best accuracy wise choice and tuning of these parameters is necessary.
\subsubsection{Prediction}
%\input{prediction}
%In this section people see failure of the trained model performing poor on general or new coming data. Questions on making prediction from the trained model or loading pre-trained model are also added here. Figure \ref{fig:prediction} shows an example question in this phase.
Our findings for the prediction category are as follows.
\paragraph*{\weka, \keras and \scikit have more problems in the prediction stage}
\weka has the highest number of problems related to prediction. The library has built-in APIs along with a GUI based work flow system. Users just need to connect different components of the workflow. We observe that despite significant attempt to make machine learning and data mining user-friendly their users face a great deal of difficulty in prediction stage. \keras and \scikit also have a higher number of problems in the prediction stage. These libraries hide almost all of the details of machine learning from the user providing abstract APIs. Though abstract APIs ease the use of ML libraries, users of abstract APIs also get suboptimal performance in prediction stage. \weka and \keras have more than 10\% questions on prediction stage and \scikit has close to 7\% questions on prediction stage. 
%\subsection{Observations}
%Some important observations from the study are given below:
%\begin{enumerate}
%	\item Libraries that use an uncommon or new format of data creates more technical debt in data preparation layer. We can observe in Figure \ref{fig:interlib} that \weka and \mllib library users face more difficulty in the data preparation stage during adapting data to the machine learning pipeline. 
%	\input{ob1}
%	As we observe in a sample question in Figure \ref{fig:ob1weka} that the user is trying to use a dataset from a well known machine learning dataset repository provided by UCI (University of California at Irvine). Usually these datasets are pre processed to do machine learning and importing these datasets can be done directly. But an user of \weka user is not able to successfully adapt the dataset to the library for training due to the failure of conversion to ARFF format needed by the library. Similarly the library Apache spark \mllib users also have a higher percentage of difficulties faced by the users at the data preparation stage. As it uses RDD format of data which is less popular to the users. Adapting the data for the library, converting from popular data formats the the format required or preferred by the library are some common problems faced by the users when the library uses less popular data formats.
%	\item  Sklearn library provides a good set of functionalities to do feature selection and feature extraction. 
%	\input{ob2}
%	For example in Figure \ref{fig:ob2sklearn} the user is facing some problem in using the built in API to select features from the data for building a model. 
%	Users also face difficulties in encoding data, cleaning data, shuffling and splitting of data, extracting features from data, data cleaning etc. The users face mainly problems related to exceptions, non satisfactory results.
%	\item Libraries that use higher abstraction create additional difficulty for users in model creation. 
%	\input{ob3}
%	For example in Figure \ref{fig:ob3} an user is trying to use the APIs provided by the library to build a model but is getting error in building the model correctly. 
%	The abstract libraries hide all the crafting techniques in building machine learning models from the users. That makes making the model interesting and easy to use to average users but can be reasons of failure to make the model working or making the best model. This problem is more common among the users of \scikit and \keras. 
%	\item Lack of rich and interactive debugging options cause a lot of difficulties 
%	in building machine learning models. When some model is throwing exception at training time, some model is not converging or learning as the iteration of training goes on, some model is not predicting well, some model creation is not correct and producing garbage results, some model is not performing well for a particular instance of a problem and a lot other problems faced by developers can ne minimized to a great extent with effective debugging options. \tensor team has attempted to add debugging options through TensorDebug \cite{tdebug}. The concept of debugging some tasks by implementing machine learning with the help of probabilistic programming is presented by the authors in \cite{chakarov2016debugging}.
%	\item \tensor has comparatively less difficulties in data preparations stage. There are some difficulties in adapting TFRecords or storing data in this format. But still \tensor provides multiple options to read and store data. And the dataset for using in the machine learning pipeline is stored as dataset of elements of same size and each element can contain on or more Tensor objects. Each Tensor object also has Type information and shape information added with it. 
%	Using Tensor object and providing functionalities to read raw data and forming dataset using Tensor objects reduce errors, adapting or data cleaning related problems. An example of how the dataset is represented as tensor from a random uniform matrix of 4*10 size is given in the following code snippet:
%	\input{tensor}
%	We see that the dataset is read and parsed as tensor by the library with type and shape information. It provides easier adapting of data as well as debugging any dataset related problem by tensor debug. \torch and \theano also uses tensors as their data structure. Although they have comparatively less problems in data preparation stage but the data adapting and loading APIs create slight difficulties compared to \tensor in these libraries. 
%	\item \tensor popularity is growing very fast since the inception of the library in November 2015. It provides some model evaluation and monitoring of the model at run time through visual interface using tensorboard, it provides some debugging functionality using tensordebug, it uses Tensor data structure to represent its data internally and flow data to different components in the pipeline. Its developers have some questions on handling sparse tensor data. And the monitoring of sparseness of the tensor at different stage is not yet supported. Analysis of sparsity of tensors at different stages of the pipeline and then optimizing the computation can be future work. And also the storing technique of different types of sparse tensors can be a great addition. Some research on the line has been proposed and presented by the authors in \cite{kjolstad2017tensor}.
%	
%	\item Converting model trained using one library and using it another library is a common problem. For example lets consider someone has trained an SVM model on a particular dataset D. The user then wants to load the model in \weka and use that for future prediction. Some libraries provide some support to convert model for using with other library but those are not always good. But some libraries dont have that support and the trained model can not be reused with other platforms.
%	\item All the library users face comparatively higher difficulty in model creation stage. Deep learning library users have comparatively more difficulty in the model creation stage. Almost 30\% of the questions asked by deep learning library users on stackoverflow where score is at least 5 is on choice of model stage. Model of choice contains topics related to model creation, selecting best model, converting model etc.
%	\item Hyperparameter tuning related questions are comparatively more to the \scikit users. Usually \scikit api designs take a lot of optional parameter. For example we see an API to create AdaBoostClassifier below with a lot of optional parameters initialized by default to None.
%	\input{sklearn}
%	And finding good value of these parameters and tuning these parameters to make the 
%	best model, avoid over-fitting are seen more among \scikit developers. 
%	There has been some github issues filed to the repository of \scikit and the reason was the user was not able to trace why the model is not showing expected accuracy. And the answer was tuning hyper parameters. For example against an issue submitted to the official repository the quick and small answer from an expert was like the following Figure \ref{fig:tune}.
%	\input{tune}
%	\item \keras a highly abstract deep learning library users get comparatively higher error at runtime. 
%	\input{keraserr}
%	For example in Figure \ref{fig:ob6} the user has built the model succesfully yet the user gets error at run time. The major reason is that building deep learning model needs to successfully connect multiple hidden layers along with the input and output layer. But using abstract libraries the user doesn't have any static analysis tool to check where the mistake has happened.
%		
%	\item \keras and Sklearn are highly abstract and hide all the details of machine learning implementations from the users. This sometimes creates some untraceable suboptimal performance in prediction. Because the user doesn't have the way to trace where the model was not functioning correctly, whether some over-fitting problem happened. For example an user has built a model successfully and got training successful with satisfactory training accuracy. But when the new data is given input to the model for prediction the prediction accuracy is very low. In most of these cases the user even doesn't have any way to trace the reason of these sub-optimal performance. So abstracting the functionalities and making more general users to practice machine learning doesn't ensure that they are doing machine learning with satisfactory success.
%	\item The libraries that are specialized for doing machine learning in the cluster have more difficulty in the choice of model phase specially in model creation. For example \mllib, \mahout are libraries to do large scale machine learning in cluster.
%	\input{mahout}
%	 The users of these libraries face higher difficulties in model creation, running model in parallel following map-reduce paradigm, selecting the appropriate model. For example in Figure \ref{fig:mahout} the user is trying to build a model to build his custom model but he has no idea on how can he create that model. The top voted answer suggested how can the person achieve his goal  by combining a multiple ideas as well as how the performance can be optimized using cluster. 
%	 \item \caffe users have problems in model creation due to the dependency of model on multiple files. To create a model successfully one needs to make a schema file in protobuf format, create a solver file and write codes in c++ or python to build the model. For example this tutorial https://medium.com/machine-learning-world/using-caffe-with-your-own-dataset-b0ade5d71233 states multiple steps needed to build a model successfully using \caffe and python. This gives us some intuition that the framework where the model depends on multiple things or there are more than one way of creating the same model creates some technical debt in the model creation phase.
%	 \item The machine learning frameworks have APIs that are very often misused. The general guideline of API design is such that it is difficult to misuse the API. But we have seen a lot of the problems faced by machine learning developers are due to using the API in an improper way. This problem happens in the APIs at almost all stages of the pipeline starting from data preparation to prediction. 
%	 \input{apimis}
%	 For example we see in Figure \ref{fig:apimis}a a question asked by a user that, his training takes much time or longer number of iterations to get a certain training accuracy. In one fit API he is able to achieve the accuracy only in 5 iterations where in other API the  user needs 60 iterations to reach the same accuracy. Everything is working fine, without any error and eventually reaching the same accuracy also. But still the user is astound by almost 12 times higher number of iterations in using the second API. And the ans in Figure \ref{fig:apimis}b suggest that the second API needs the data to shuffled properly before passing to the API in every iteration. And changing only that part solved the performance problem.
%	 
%	 This kind of API misuse is very common in machine learning API at all stages. It causes problems on failure to find important features, properly preparing the dataset, performance, over-fitting, suboptimal prediction performance, error, warnings etc. 
%	 \item Shape mismatch of tensors at different layers is also a common problem among the libraries that use tensors or matrices. This problem is seen more commonly in deep learning library. For example when tensors pass from layer $i$ to layer $j$ in the network then there should be some size compatibility otherwise it can raise exception during training and even it can fail at the very starting of the runtime. 
%	 \input{shape}
%	 For example we see in Figure \ref{fig:shape} a sample question on shape mismatch. 
%	 \item Type mismatch is also a common problem faced by developers. The training stops due to this type mismatch problem. 
%	 \input{type}
%	 For example Figure \ref{fig:type} shows a question on type mismatch. 
%\end{enumerate}




==> libanalysis.tex <==
%\input{intracharts}
%\input{intratable}
%\section{Analysis and Results}
%\label{sec:evaluation}

\subsection{Intra-Library Analysis}
\label{sec:intra-library}

%\input{interold}
In this section, we 
% discuss our study results on the problems raised in the \sof posts for each library individually.
%We 
discuss the potential strengths and weaknesses of each library 
w.r.t. our classification in \figref{fig:classes}.
% at different stages and (sub)categories. 
The statistics are shown in \tabref{tbl:cat} and \tabref{tbl:subcat}. 

\input{intranew}

\subsection{Inter-Library analysis}
\label{sec:inter-library}

%\input{librarycatchart} 

In this section, we  present our analysis and observations across ML libraries. 
%In the following section, we present the analysis results that focus on a single ML library at-a-time. 
%
% In this section we present the results of our observation of developer behaviors
% in using different machine learning frameworks \cite{stages}. We also classify
% the problems faced in each stage into different categories.
%
%
We study the strengths and weaknesses of different ML libraries 
in terms of each of the top-level categories defined in \figref{fig:classes}.
% We study different libraries and see the strong and weak part of 
% different libraries at different stages of machine learning in terms 
% of developers difficulty. 
% The distributions of the percentages of questions over stages of all 
% libraries are shown in the heatmap in \tabref{tbl:cat} and \tabref{tbl:subcat}.
The distribution of questions over stages of all 
libraries are shown in \tabref{tbl:cat} and \tabref{tbl:subcat}.

%\figref{fig:interlib}. 

%\input{interlibanalysis}

\input{internew}

\input{misuses}

\input{inter-group}


==> librarycatchart.tex <==
\begin{figure}[t]
	\includegraphics[width=\columnwidth]{interlibstudy}
	\caption{Distribution of questions of different libraries in different categories}
	\label{fig:comparelibs}
\end{figure}

==> macros.tex <==
% $Id: macros.tex,v 1.55 2014/03/28 18:10:44 csgzlong Exp $

% \newcommand{\notes}[2]{\textbf{note(#1): #2}}
% \newcommand{\todos}[2]{\textbf{TODO(#1): #2}}

% Use to temporarily disable all notes and todos
\newcommand{\notes}[2]{}
\newcommand{\todos}[2]{}


\usepackage{xcolor}
\usepackage{relsize}
\usepackage{listings}
\usepackage{multirow}
\usepackage{pifont} % for \cmark and \xmark
\usepackage{framed}
\usepackage{balance} % to balance the bibliography



\renewcommand{\ttdefault}{pcr}
\lstset{
language=Java,                            % Code langugage
basicstyle=\ttfamily,                     % Code font, Examples: \footnotesize, \ttfamily
%keywordstyle=\color{OliveGreen}\bfseries, % Keywords font ('*' = uppercase)
% keywordstyle=\bfseries,
keywordstyle=\bfseries\color{dkgreen},
commentstyle=\color{gray},                % Comments font
numbers=left,                             % Line nums position
% numberstyle=\tiny,                        % Line-numbers fonts
stepnumber=1,                             % Step between two line-numbers
numbersep=5pt,                            % How far are line-numbers from code
backgroundcolor=\color{lightlightgray},   % Choose background color
frame=none,                               % A frame around the code
tabsize=2,                                % Default tab size
captionpos=b,                             % Caption-position = bottom
breaklines=true,                          % Automatic line breaking?
breakatwhitespace=false,                  % Automatic breaks only at whitespace?
showspaces=false,                         % Dont make spaces visible
showtabs=false,                           % Dont make tabs visible
%columns=flexible,                        % Column format
}

\newcommand{\FIGCODEFONT}{\linespread{1}\ttfamily}
% \newcommand{\FIGCODEFONT}{\relsize{-2}\ttfamily}
\newcommand{\FIGCODELIBFONT}{\relsize{-6}\ttfamily}

\newcommand{\etal}{\textit{et al.}}

\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\tableref}[1]{Table~\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\secref}[1]{\S\ref{#1}}
\newcommand{\lineref}[1]{line~\ref{#1}}
\newcommand{\linesref}[2]{lines~\ref{#1}-\ref{#2}}
\newcommand{\lstref}[1]{Listing~\ref{#1}}

\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}

\newcounter{NumFindings}
\stepcounter{NumFindings}
\newcommand{\findings}[2]{%
\begin{framed}%
	% \vspace{-0.75em}%
	\noindent\begin{minipage}{\linewidth}%
		{\bf{Finding \arabic{NumFindings}}}: #1 \\
		{\bf{Implication}}: #2
	\end{minipage}%
	% \vspace{-0.75em}%
\end{framed}%
\stepcounter{NumFindings}
}


==> motiv.tex <==
\begin{figure}[t]
	\includegraphics[width=\columnwidth]{motiv}
	\caption{In machine learning it often appears that the user doesn't have the clue after training the model using library where did the wrong happen (Details code snippet omitted)}
	\label{fig:motiv}
\end{figure}

==> ob1.tex <==
\begin{figure}[t]
	\includegraphics[width=\columnwidth]{ob1}
	\caption{Problem faced by an user to import popular CSV format data into ARFF to use in training with \weka.}
	\label{fig:ob1weka}
\end{figure}

==> ob2.tex <==
\begin{figure}[ht]
	\includegraphics[width=\columnwidth]{ob2feature}
	\caption{Feature selection difficulty in using built-in feature selection APIs by \scikit}
	\label{fig:ob2sklearn}
\end{figure}


==> ob3.tex <==
\begin{figure}[t]
	\includegraphics[width=\columnwidth]{ob3sklearn}
	\caption{An example question on \scikit showing abstraction can create more confusion in machine learning libraries}
	\label{fig:ob3}
\end{figure}

==> popular.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{popular}
	\caption{Popular Machine learning libraries}
	\label{fig:popular}
\end{figure}

==> prediction.tex <==
\begin{figure}[t]
	\includegraphics[width=\columnwidth]{prediction}
	\caption{A stackoverflow question on hyper prediction phase of using a library}
	\label{fig:prediction}
\end{figure}

==> repu2.tex <==
\begin{figure}[ht]
	\includegraphics[width=\columnwidth]{boxplot}
	%\vspace{-1.5em}
	\caption{Box plot showing the reputation of the reputation of users asking questions about different ML libraries}
	\label{fig:boxplot}
\end{figure}

==> tensor.tex <==
\begin{lstlisting}[language=Python]
dataset1 = tf.data.Dataset.from_tensor_slices(tf.random_uniform([4, 10]))
print(dataset1.output_types)  
# ==> "tf.float32"
print(dataset1.output_shapes) 
# ==> "(10,)"

\end{lstlisting}

==> training.tex <==
\begin{figure}[t]
	\includegraphics[width=\columnwidth]{training}
	\caption{A Stack Overflow question on training phase of using a library}
	\label{fig:training}
\end{figure}

==> type.tex <==
\begin{figure}[t]
	\includegraphics[width=\columnwidth]{type}
	\caption{An example question showing type mismatch problem that can cause failure of training at any step of the iterations.}
	\label{fig:type}
\end{figure}
